A Convergence Theory Towards Practical Over-parameterized Deep Neural Networks

Deep neural networks' remarkable ability to correctly fit training data when optimized by gradient-based algorithms is yet to be fully understood. Recent theoretical results explain the convergence for ReLU networks that are wider than those used in practice by orders of magnitude. In this work, we take a step towards closing the gap between theory and practice by significantly improving the known theoretical bounds on both the network width and the convergence time. We show that convergence to a global minimum is guaranteed for networks with widths quadratic in the sample size and linear in their depth at a time logarithmic in both. Our analysis and convergence bounds are derived via the construction of a surrogate network with fixed activation patterns that can be transformed at any time to an equivalent ReLU network of a reasonable size. This construction can be viewed as a novel technique to accelerate training, while its tight finite-width equivalence to Neural Tangent Kernel (NTK) suggests it can be utilized to study generalization as well.

==> discussion.tex <==
 \subsection{Discussion}
%   Add a table with:
%   \begin{itemize}
%     \item Minimal width dependency on n,L. 
%      \item error probability 
%      \item assumptions on data
%      \item number of iterations (linear convergence rate): Allen- $O\left(\frac{n^6L^2}{\delta^2\log(\frac{1}{\varepsilon})})\right)$
%      \item NTK related size.
%      \item learning rate(?)
%      \item possibly we are not bounded to $y=O(1)$ while Allen does?
%  \end{itemize}
% \begin{table}[t]
%   \centering
%   \setlength{\tabcolsep}{2pt}
%   \resizebox{\linewidth}{!}{
%   \scalebox{0.01}{
%   \begin{tabular*}{0.5\textwidth}{l @{\extracolsep{\fill}} c c c c c}
%     \toprule
%     Work & Iterations & Neurons & Probability & Learn-rate & Remarks \\
%     \midrule
%     Du~\citep{du2019gradient} & $O\left(\frac{1}{\eta \lambda_0} \log\frac{1}{\varepsilon}\right)$ & $\Omega \left( \frac{n^6}{\lambda_0^4p^3 }\right)$              & $p$ & $O\left( \frac{\lambda_0}{n^2}\right)$ & $\lambda_0^{-1}=\textrm{poly}\left(2^{O(L)},n,d \right)$ ,  \textrm{binary,smooth activations}  \\
%     Allen-Zhu~\citep{allen2019convergence} & $\Theta\left(\frac{n^6L^2}{\delta^2\log(\frac{1}{\varepsilon})})\right)$ & $\Omega \left(\frac{n^{24}L^{12}d\log^5m}{\delta^8} \right)$              & $O\left( \exp\paren{-\log^2 m}\right)$ & $\Theta\left(\frac{\delta^9}{n^{28}\log^5m L^{14}}  \right)$   \\
%     Zhu~\citep{zou2018stochastic} & $O\left( n^8L^9\delta^{-2}\right)$ & $\Omega \left( \frac{n^{26}L^{38}}{\delta^8}   \right)$ & $p$ & $O\left(n^{-29} L^{-47}\delta\right)$ & binary classification  \\ \midrule
%     Ours & $O\left(\frac{n^4}{d^2} \log\frac{1}{\varepsilon}\right)$ & $\Omega\left(\max\paren{n^2,n^{\frac{2}{3}}d^{\frac{4}{3}}\sqrt{\ell_1}}\right)$ & $O\left(\exp(-\Omega(\sqrt{m})\right)$ & $\Theta\left(\frac{d^4}{n^8L}\right)$  \\
%     \bottomrule
%   \end{tabular*}
%   } }
% %  \caption{caption}
% %mention in caption that Du's activation are only smooth.
%   \label{table:EfficientNet}
% \end{table}


% \begin{table}[t]
%   \centering
%   \setlength{\tabcolsep}{2pt}
%   \resizebox{\linewidth}{!}{
%   \scalebox{0.01}{
%   \begin{tabular*}{0.5\textwidth}{l @{\extracolsep{\fill}} c c c c c}
%     \toprule
%     Work & $O\left(\#\textrm{Iterations}\right)$ & $\Omega\left(\#\textrm{Neurons}\right)$ & $O\left(\textrm{Probability}\right)$ & $\Theta\left(\textrm{Learn-rate}\right)$ & Remarks \\
%     \midrule
%     Du~\citep{du2019gradient} & $ \frac{1}{\eta \lambda_0} \log\frac{1}{\varepsilon}    $ & $\frac{n^6}{\lambda_0^4p^3 }    $              & $p$ & $  \frac{\lambda_0}{n^2}    $ & $\lambda_0^{-1}=\textrm{poly}\left(2^{O(L)},n,d\right)     $ ,  \textrm{binary,smooth activations}  \\
%     Allen-Zhu~\citep{allen2019convergence} & $   \frac{n^6L^2 \log(\frac{1}{\varepsilon})}{\delta^2}    $ & $\frac{n^{24}L^{12}d\log^5m}{\delta^8}     $              & $  \exp\paren{-\log^2 m}    $ & $   \frac{\delta^9}{n^{28}\log^5m L^{14}}      $   \\
%     Zhu~\citep{zou2018stochastic} & $  \frac{n^8L^9}{\delta^{2}}    $ & $ \frac{n^{26}L^{38}}{\delta^8}       $ & $p$ & $\frac{\delta}{ n^{29} L^{47}}    $ & binary classification  \\ \midrule
%     Ours & $ \frac{n^4}{d^2} \log\frac{1}{\varepsilon}    $ & $  \max\paren{n^2,n^{\frac{2}{3}}d^{\frac{4}{3}}\sqrt{\ell_1}}    $ & $ \exp(-\Omega(\sqrt{m})    $ & $   \frac{d^4}{n^8L}    $  \\
%     \bottomrule
%   \end{tabular*}
%   } }
% %  \caption{caption}
% %mention in caption that Du's activation are only smooth.
%   \label{table:EfficientNet}
% \end{table}


% \begin{table}[ht]
% \centering
% %  \begin{center}
%   %\setlength{\tabcolsep}{2pt}
%   %\resizebox{\linewidth}{!}{
%   %\scalebox{0.01}{
% %   \begin{tabular*}{0.5\textwidth}{l @{\extracolsep{\fill}} c c c c c}
%   %\begin{tabular}%{\textwidth}
%     \caption{bla}
%   \begin{tabular}{|p{1.3cm} p{2.4cm} p{2.7cm} p{1.4cm} p{2cm} p{4.5cm}|}
%   %{1\textwidth}
%   %{l @{\extracolsep{\fill}} 
%   %{l c c c c c}
%     %\toprule
%     Work & 
%     $\Omega\left(\#\textrm{Neurons}\right)$ & $O\left(\#\textrm{Iters}\right)$ & $O\left(\textrm{Prob}\right)$ & $\Theta\left(\textrm{Step}\right)$ & 
%     Remarks \\
%     %\midrule
%     \hline
%     Du\citep{du2019gradient} &
%     $\frac{n^6}{\lambda_0^4p^3 }    $&
%     $ \frac{1}{\eta \lambda_0} \log\frac{1}{\varepsilon}    $ &
%     $p$ & 
%     $\frac{\lambda_0}{n^2} $ & \small$\lambda_0^{-1}=\textrm{poly}\left(2^{L},n\right),\textrm{BC,SA}$\\%binary-class, smooth activations
%     %\hline
%     Allen\citep{allen2019convergence} & 
%     $\frac{n^{24}L^{12}d\log^5m}{\delta^8}$ & 
%     $   \frac{n^6L^2 \log(\frac{1}{\varepsilon})}{\delta^2}    $ &
%     $  e^{-\log^2 m}    $ &
%     $   \frac{\delta^9}{n^{28}\log^5m L^{14}}  $ & --  \\
%     Zou\citep{zou2018stochastic} & 
%     $ \frac{n^{26}L^{38}}{\delta^8}       $ &
%     $  \frac{n^8L^9}{\delta^{2}}    $ &
%     $p$ & $\frac{\delta}{ n^{29} L^{47}}    $ &
%     binary classification  \\ \midrule
%     \textbf{Ours} & 
%     \small$ \Omega{\paren{n^2 d L} }$ &
%     \small$ n L^{1/2}d^{1/4}\log\paren{\frac{m n}{\varepsilon}} $ &
%     $ e^{-\sqrt{m}} $ &
%     $ \frac{d^{3/4}}{m^2n L^{3/2}} $ & $L\in\paren{\Omega(\log n),O(n^2)}$ \\
%     %\bottomrule
%     % \textbf{Ours} & 
%     % \small$ \Omega{\paren{n^2 d_y^2 d_x L} }$ &
%     % $ n L^{1/2}d_x^{1/4} d_y^{3/4}\log\paren{\frac{m n d_y}{\varepsilon}} $ &
%     % $ e^{-\sqrt{m}} $ &
%     % $ \frac{d_x^{3/4}d_y^{1/4}}{m^2n L^{3/2}} $ & $L\in\paren{\Omega(\log n),O(n^2)}$ \\
%     % %\bottomrule
%   \end{tabular}
%   %} %}
%   \caption{BC-binary classification, d-input dimension SA-smooth activations}
% %mention in caption that Du's activation are only smooth.
%   \label{table:theo_comparison}
% %    \end{center}
% \end{table}
%  \asaf{changes 'our's sizes after changes in theorem 4, and add to table stuff from the analytic-activation paper.}
% \begin{table}[ht]
% \centering
% %  \begin{center}
%   %\setlength{\tabcolsep}{2pt}
%   %\resizebox{\linewidth}{!}{
%   %\scalebox{0.01}{
% %   \begin{tabular*}{0.5\textwidth}{l @{\extracolsep{\fill}} c c c c c}
%   %\begin{tabular}%{\textwidth}
%     \caption{bla}
%   \begin{tabular}{|p{1.3cm} p{2.4cm} p{1.7cm} p{1.4cm} p{2cm} p{5cm}|}
%   %{1\textwidth}
%   %{l @{\extracolsep{\fill}} 
%   %{l c c c c c}
%     %\toprule
%     Work & 
%     $\Omega\left(\#\textrm{Neurons}\right)$ & $O\left(\#\textrm{Iters}\right)$ & $O\left(\textrm{Prob}\right)$ & $\Theta\left(\textrm{Step}\right)$ & 
%     Remarks \\
%     %\midrule
%     \hline
%     Du\citep{du2019gradient} &
%     $\frac{n^6}{\lambda_0^4p^3 }    $&
%     $ \frac{1}{\eta \lambda_0} \log\frac{1}{\varepsilon}    $ &
%     $p$ & 
%     $\frac{\lambda_0}{n^2} $ & \small$\lambda_0^{-1}=\textrm{poly}\left(2^{O(L)},n\right),\textrm{BC,SA}$\\%binary-class, smooth activations
%     %\hline
%     Allen\citep{allen2019convergence} & 
%     $\frac{n^{24}L^{12}d\log^5m}{\delta^8}$ & 
%     $   \frac{n^6L^2 \log(\frac{1}{\varepsilon})}{\delta^2}    $ &
%     $  e^{-\log^2 m}    $ &
%     $   \frac{\delta^9}{n^{28}\log^5m L^{14}}  $ & --  \\
%     Zou\citep{zou2018stochastic} & 
%     $ \frac{n^{26}L^{38}}{\delta^8}       $ &
%     $  \frac{n^8L^9}{\delta^{2}}    $ &
%     $p$ & $\frac{\delta}{ n^{29} L^{47}}    $ &
%     BC  \\ \midrule
%     Ours & 
%     \small $nd\log({nd})$ &
%     $ \frac{n^4}{d^2} \log\frac{1}{\varepsilon} $ &
%     $ e^{-\sqrt{m}} $ &
%     $ \frac{d^4}{n^8L}$ & --  \\
%     %\bottomrule
%   \end{tabular}
%   %} %}
%   \caption{comparison deep networks overparameterization}
% %mention in caption that Du's activation are only smooth.
%   \label{table:theo_comparison}
% %    \end{center}
% \end{table}




% \begin{thm} \label{thm:linear_rate_convergence}
%  Suppose the network in \autoref{sec:preliminaries} with width $m=\Omega{\paren{n^2 d_y^2 d_x L} }    
%  $ and depth $L\in\paren{\Omega(\log n),O(n^2)}$ is trained by gradient-descent with learning rate $\eta=\Theta\paren{\frac{d_x^{3/4}}{m^2 n L^{3/2}d_y^{1/4}}}$, 
%  then with probability of at least $1 - \exp(-\Omega(\sqrt{m}))$ over the random initialization,
%  it reaches $\epsilon$-error in $T=O\paren{n L^{1/2}d_x^{1/4} d_y^{5/4}\log\paren{\frac{n^3 d_y^3 d_x L}{\varepsilon}}}$ iterations.
 
 %eta=\Theta\left(\frac{d^4}{n^8L}\right)$
%T= O\left(\frac{n^4}{d^2} \log\frac{1}{\varepsilon}\right)
%m=\Omega\left(\max\braces{n^2,n^{\frac{2}{3}}d^{\frac{4}{3}}}\right)
%\end{thm}

==> experiments_old_v0.tex <==

\section{Experiments} \label{sec:experiments}
In this section, we provide empirical validation for the theoretical results on different datasets. In order to compare the proposed approach with the traditional ReLU one, we have implemented our concept with Gated ReLU as presented in Figure (\ref{fig:network_blocks}) in a fully connected (FC) network with different numbers of layers and channels per layer, and have compared the results with the exact same architecture using regular ReLU.
% We address the following points:
% \begin{itemize}
%     \item How does the number of layers and channels impact the performance of our method ?
%     \item How close to the theory are the practical hyper-parameters such as learning rate, number of steps, final MSE... ?
%     \item Is our method limited to regression or can be extended to classification ?
%     \item Can our method be an alternative to ReLU without any or just a few computational overhead?
% \end{itemize}
We start with an experiment on a 'real-world' regression dataset, move to a synthetic dataset in order to have freedom to choose hyper-parameters such has dimensional embedding and number of data-samples, and then show that this idea can also be applied in classification. In both cases, we try to vary the number of channels and layers to observe their impact on the convergence. 
% \subsection{Implementation for twice faster training and inference}
% The implementation of Gated ReLU is straightforward, and is described in Fig. \ref{fig:network_blocks}. It consists of two networks in parallel, initialized independently, while the second (auxiliary) network controls the ``gates'' replacing the ReLU in the main network. The auxiliary network is not a strict copy of the main network since this would imply to multiply the computational complexity of the inference by 2. Instead, for every convolution layer in the main network that requires $(m\times m)$ operations, we associate to the auxiliary network a low rank approximation consisting of a succession of two FC layers with respective sizes $(m\times r)$ and $(r\times m)$ where $r<<m$ is chosen to be fixed (in practice $r=200$). In this setting, instead of using $m^2$ operations for every layer as it would be required if the auxiliary network would be similar to the main one, we have $2rm$ operations, that is only $10\%$ of the computations required by a regular FC network given the choice of $r$ and $m$. Since the gates depend only on the output of the auxiliary network, and the theoretical and empirical ratio of such opened gates is 0.5, after we have ran an example inside the auxiliary network, we can know in advance what channels have their output activated by the gates, and avoid to compute the ones whose associated gate is closed. In this setting, the main network requires just $50\%$ of the FLOPS required by a single ReLU network. In total, the computational complexity required by our method is $60\%$ of the one required by its ReLU counterpart, $10\%$ required by the auxiliary network, and $50\%$ by the main network given the fact that our matrix multiplications are sparse. Training with a lookup table allows further reduction to around $50\%$, since the open Gated Relu are already known in advance, by definition.
\subsection{Regression}
\paragraph{SGEMM dataset}
We choose the SGEMM GPU kernel performance dataset~\citep{nugteren2015cltune}, available online\footnote{\url{https://archive.ics.uci.edu/ml/datasets/SGEMM+GPU+kernel+performance}} with $241,600$ samples. This data set measures the running time of a matrix-matrix product $AB = C$, where all matrices have size $(2048 \times 2048)$, using a parameterizable SGEMM GPU kernel with $241,600$ possible parameter combinations. We build a network using 10 FC layers with 4096 features. For both Gated ReLU and Regular ReLU experiments, we use the same initialization, and structure. 
We train our networks with different learning rates, both for the Gated and regular ReLU, and present results in Figures \ref{fig:train_loss_cst} and \ref{fig:train_loss_relu}. The chosen learning rate is the one that lead to a stable training and does not diverge or oscillate too much. We can see that our method converges faster and is more stable allowing  higher learning rate. While our method can converge with a learning rate of $10^{-3}$, the maximum learning rate that would not lead to divergence for regular Relu is $10^{-4}$. When multiplying this latter by two, we can already see the training loss getting unstable.  In Figure \ref{fig:train_loss_sgemm3}, we present the evolution of the loss when using same learning rate for both regular and Gated ReLU's. We can observe that the Gated ReLU network has a more stable training, meaning a monotone loss decrease, and converges faster to a lower MSE.

In order to explain the reason for the fact that our method allows a higher learning rate, for every step, we compute the MSE between the gradients of the current and previous step, and present this difference as function of a step in Figure \ref{fig:train_loss_grad} both for our method and regular ReLU when using a stable learning rate for both methods of $10^{-4}$. The higher this difference, the less stable is the training, since it would imply that the gradients change a lot during the training. In Figure \ref{fig:successive_relu_hamming}, we present the mean hamming distance between the activation patterns of the ReLU at two consecutive epochs. For this, we select a subset of input data, and record the pattern of the activated ReLU for the network at epoch $e$ and $e+1$, and compute the average hamming distance between them on all images, layers, and neurons in the network. W can observe that as the training evolves, this activation pattern for ReLU network changes more and more, while it does not vary at all (by definition) for our Gated ReLU, that could explain the fact that the training is more stable, and that the gradients in our network vary less than the ones in the ReLU one. As predicted by Theorem \ref{thm:NTK}, we can observe that, unlike regular ReLU, this difference does not increase along the training and even get smaller, leading to a more stable training and allowing higher learning rates. 

Finally, we show the impact of the number of channels and layers in Figure \ref{fig:train_loss_sgemm2}. As can be seen, it seems that our method performs better with deeper network than with shallower wider ones.
%We also use the highest possible learning rate that does not lead to divergence. For Gated ReLU; the learning rate is $7\cdot10^{-5}$ while for regular ReLU, the learning rate used is $2\cdot10^{-5}$.  In addition, we also compare the convergence of our network using the same learning rate as the regular ReLU one (even though the latter is not optimal for our metehod). We train the regression for 600 epochs, using SGD with Nesterov momentum set to $0.9$. Figure \ref{fig:train_loss_sgemm} shows the evolution of the MSE as a function of epochs. We can see that using gated Relu leads to faster convergence, but also to a lower MSE, not only using the maximum possible learning rate, but also using a lower learning rate that leads to more stable convergence. The fact that we do not reach zero error is because we do not train the network until full convergence, as the theory shows that this would require a significantly higher number of epochs. In addition, we show the impact of the number of channels and layers in Figure \ref{fig:train_loss_sgemm2}. As can be seen, it seems that our method performs better with deeper network than with shallower wider ones.



\begin{figure}[h]
    \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
            \includegraphics[width=\textwidth]{figures/train_err_sgemm_cst.pdf}
            \caption{Gated ReLU}
            \label{fig:train_loss_cst}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
         \centering
            \centering
    \includegraphics[width=\textwidth]{figures/train_err_sgemm_relu.pdf}
    \caption{Regular  ReLU}
    \label{fig:train_loss_relu}
    \end{subfigure}
    \caption{MSE as a function of epochs on SGEMM dataset}
\end{figure}



\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
            \includegraphics[width=\textwidth]{figures/train_err_sgemm_lr_1e2.pdf}
        \caption{lr=$10^{-2}$}
    \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
            \includegraphics[width=\textwidth]{figures/train_err_sgemm_lr_1e3.pdf}
        \caption{lr=$10^{-3}$}
    \end{subfigure}
         \begin{subfigure}[b]{0.32\textwidth}
         \centering
            \includegraphics[width=\textwidth]{figures/train_err_sgemm_lr_7e4.pdf}
        \caption{lr=$7\cdot 10^{-4}$}
    \end{subfigure}
    \caption{MSE as a function of epochs for regular and Gated ReLU on SGEMM dataset. Our method converges faster to a smaller MSE}
    \label{fig:train_loss_sgemm3}
\end{figure}


\begin{figure}[h]
    \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
    \includegraphics[width=\textwidth]{figures/train_err_sgemm_grad.pdf}
    \caption{Average temporal difference of gradient for regular and Gated ReLU on SGEMM dataset}
    \label{fig:train_loss_grad}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
         \centering
    \includegraphics[width=\textwidth]{figures/activation_relu.pdf}
    \caption{Average temporal hamming distance between successive binary ReLU's activation pattern}
    \label{fig:successive_relu_hamming}
    \end{subfigure}
    \caption{Evolution of gradients and activation patterns}
\end{figure}


\begin{figure}[!tbp]
  \centering
  \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/train_err_synt.pdf}
    \caption{MSE as a function of epochs for regular and Gated ReLU on synthetic dataset}
    \label{fig:synthetic_loss}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/train_err_sgemm_different_sizes.pdf}
    \caption{MSE as a function of epochs, number of kernel and layers for Gated ReLU on SGEMM.}
    \label{fig:train_loss_sgemm2}
  \end{minipage}
\end{figure}





\begin{figure}[!tbp]
  \centering
  \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/theory_graph.pdf}
    \caption{MSE vs epochs for theoretic and sub-theoretic widths of a $4$-layers network.}
    \label{fig:theory_graph}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{figures/train_err_cifar10.pdf}
    \caption{Training loss as a function of epochs for regular and custom ReLU on CIFAR-10}
    \label{fig:train_loss_cifar}
  \end{minipage}
\end{figure}



\paragraph{Synthetic Dataset}
In this experiment, we generate a regression dataset using a explicit functional. Given a input vector $x\in\mathbb{R}^n$, the following mapping is applied: 
$$
f(x)=\sum_i x_{n-i}\left(\log{\left(|x_i|\right)\left(\cos(x_i)+x^3\sin(x)\right)}+\sqrt{|x|}\right)
$$
We choose a setting where the dimensionality of the input is 200, and generate 100.000 samples. We use the same architecture as in the previous paragraph, a 10 layer fully connected network with 4096 features in each layer. We try to compute the average MSE loss for several learning rates, both for our Gated ReLU and the regular ReLU. results are presented in Fig. \ref{fig:synthetic_loss}. Again we can see that not only our method has a more stable training and allows higher learning rates, but also, converges to zero MSE while regular ReLU does not reach it.
In addition, to test how tight is the theoretical bound $m=n^2L$ presented in \ref{table:theo_comparison}, we generate 100 examples, and we build a 2-layers network with $m\approx n^2L$ to have similar settings as in our theory, and two other networks with lower $m$, and present the results in \ref{fig:theory_graph}. As we can see, our bound is tight, since we do not reach zero error when taking smaller number of features $m$.

\subsection{CIFAR-10}
We also implement our method on CIFAR-10 dataset.
For all of our experiments, we train our networks on CIFAR-10 dataset, from which every $(32\times 32 \times 3)$ input image is converted to a $3072$-dimensional normalized vector. We initialize the FC network as described in Section~\ref{sec:preliminaries}. Every exeriment is conducted with the same hyper parameters. We train both networks with learning rate $10^{-4}$. %Even though the Cifar dataset is a classification dataset, where the conventional loss is computed as a cross entropy between the softmax of the output logits and the true target, in our setting, 
We express the problem as a regression one and use a mean squared error between the output logits and the one-hot vector encoding the correct class.  Results are presented in the below table:

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
         Network architecture & train error with regular ReLU & train error with Gated Relu \\ \hline
         6 layers, 10k channels & 0.48 & 0.02  \\ \hline
         7 layers, 10k channels & 0.27 & 0.01  \\ \hline
         4 layers, 15k channels & 0.75 & 0.03  \\ \hline
    \end{tabular}
    \caption{Training error for regular and Gated ReLU's on Cifar 10}
    \label{tab:experiment}
\end{table}

In Figure \ref{fig:train_loss_cifar}, we show the evolution of the training loss as a function of epoch for Gated and Regular ReLU on CIFAR 10 using a FC network with 4 layers and 15k channels. We can see that the training loss of the Gated ReLU network converges to zero much faster that the one with Regular ReLU.
% \begin{wrapfigure}[14]{r}{0.5\textwidth}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/train_err_cifar10.pdf}
%     \caption{Training loss as a function of epochs for regular and custom ReLU on CIFAR-10}
%     \label{fig:train_loss_cifar}
% \end{wrapfigure}
% \asaf{If we put a table (2) instead of graph it can contain: 1. test error (once, so we can focus on train-error in graphs. 2. FLOPS, so no one will miss the ~50 percent improvement :) \\
% Synthetic - better \citep something on the selected function. Also, not sure what is the point behind the current experiment (let's discuss).}
\subsection{Discussion}
Referring to table \ref{table:theo_comparison}, we can compute the theoretical number of neurons and learning rate required to reach zero accuracy. We can see that the learning rate we used in practice both for Cifar and SGEMM experiments is higher that the theoretical one and that the number of neurons per layer is much smaller that the theoretical one. Yet, in CIFAR, it converged to a zero training error. We also notice that the pratical maximum learning rate is higher that the one of a regular ReLU network. The fact that the per example activation patterns stay constant along the training process allows the gradient to vary a very little, leading thus to a more stable training.


==> experiments_old_v1.tex <==

\section{Experiments} \label{sec:experiments}
In this section, we provide empirical validation for our theoretical results, as well as further testing on complementary setups. We wish to answer the following questions:
\begin{enumerate}
    \item \textit{Is the theoretical guarantee of Theorem~\ref{thm:linear_rate_convergence} tight, or can it be further improved?}
    % \item \textit{How do the two networks compare in practical setups?}%when trained over real-world datasets?}
        \item \textit{How well do GReLU networks compared to ReLU networks in practical scenarios?}
    \item \textit{What is the difference between the training dynamics of GReLU and ReLU when optimized with gradient-descent?}
\end{enumerate}
The next sections are dedicated to discuss those questions.
For a fair comparison, we select networks with the same initialization described in Section~\ref{sec:preliminaries}, width and depth, trained by gradient descent with a constant learning rate for each train. The term MSE refers to the \textit{sum} of squared errors described in~(\ref{notation:loss}).
Since the theory covers general setups, it often provide conservatively small learning rates to fit all setups, while in practice larger values can be utilized for faster convergence. Therefore, we experiment with changing learning rates according to the tasks. Also, in all experiments we optimize with batch gradient-descent due to hardware constraints. We pick the largest possible batch size per experiment for both variants.
%\asaf{mention somewhere SGD, fixed lr.}
%The following sections will deal 
\begin{figure}[h]
    \centering
     \begin{subfigure}[b]{0.32\textwidth}
        \centering
     \includegraphics[width=\textwidth]{figures/theory_graph.pdf}
    \caption{MSE vs epochs for theoretic and sub-theoretic widths of a\\ $4$-layers network}
    \label{fig:theory_graph}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
    \includegraphics[width=\textwidth]{figures/train_err_sgemm_grad.pdf}
    \caption{Average temporal difference of gradients for ReLU and GReLU for SGEMM dataset}
    \label{fig:train_loss_grad}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
    \includegraphics[width=\textwidth]{figures/activation_relu.pdf}
    \caption{Average Hamming distance of successive ReLU activations patterns for SGEMM dataset}
    \label{fig:successive_relu_hamming}
    \end{subfigure}
%    \caption{Evolution of gradients and activation patterns}
\end{figure}
\subsection{Lower Trainability Bound}
To answer \textbf{question 1}, we test both networks on a synthetic dataset, in order to control the number of examples and their dimension to fit the theory with GPU memory constraints. 
We generate a regression problem with the following complex version of the Ackley function~\citep{potter1994cooperative},
$$
y_i=\sum_{d'=1}^d x_{i,d-d'}\left(\log{\left(|x_{i,d'}|\right)\left(\cos(x_{i,d'})+x^3\sin(x_{i,d'})\right)}+\sqrt{|x_{i,d'}|}\right)~~,~~i=1,\dots, n
$$
We generate $\paren{n,d}=\paren{100,200}$ random vectors and labels, and use $4$-layers networks for both ReLU and GReLU, with changing widths. The results of the different runs appear in Figure~\ref{fig:theory_graph}. First, we set $m$ based on the order of the theoretical bound in theorem~\ref{thm:linear_rate_convergence}, $m=n^2L$. 
As both networks converge to a zero error, we decrease $m$ until reaching points where each of the networks do not converge. Interestingly, both networks behave similarly for different orders of $m$, and do not converge for lower orders of width, i.e. $m=\paren{n^2L}^p, p<1$ and $m=n L$. 
As our theory guarantees convergence for \textit{any} dataset that satisfies Assumptions~\ref{assum:input}-\ref{assum:labels}, these results provide empirical support for our theorem being tight. We note that training with significantly smaller learning rates than the ones tested and corresponding impractically longer convergence times, narrower networks would possibly converge as well. Also, while we focus on fully-connected networks, 
modern architectures like convolutional networks~\citep{he2016identity} were shown to converge with smaller widths (channels) for specific tasks.
\subsection{Comparison Over Practical Scenarios}
In this section we train and evaluate both networks with practical learning rates, widths and depths over the following two popular datasets:\\ %We aim to
% In all experiments we select networks with the exact same width and depth for fair comparison, trained by gradient descent with fixed learning rates. Since the theory covers general setups, it often provide conservatively small learning rates to fit them all, while in practice larger values can be utilized for faster convergence. Therefore, we experiment with changing learning rates according to tasks. Also, in all experiments we optimize with batch gradient-descent due to hardware constraints. We pick the largest batch size per experiment for both variants.
% it tends to conservative regarding the maximal learning rates, while in practice larger values can be utilized for faster convergence. The selected datasets:\\
\textbf{SGEMM}
%We start with 
the well known CPU kernel-performance regression dataset\footnote{\url{https://archive.ics.uci.edu/ml/datasets/SGEMM+GPU+kernel+performance}}~\citep{nugteren2015cltune}. It contains $n=241,600$ samples of dimension $d=18$, measuring CPU runtime of matrix products.\\
\textbf{CIFAR-10} the popular image classification dataset, with $n=50,000$ and $d=32\times 32 \times 3=3072$.
% We  transform it to a scalar regression task by calculating the squared error between its output logits and the one-hot $10$ dimensional vector encoding its labels. \\
We  transform each classification to a scalar regression by calculating the squared loss between the one-hot $10$ dimensional vector encoding its correct label and the output logits of the network. \\
These datasets offer high diversity with different domains, input dimensions and structures. They were selected to test both networks over more practical scenarios than the previous synthetic dataset.
% We also implement our method on CIFAR-10 dataset.
% For all of our experiments, we train our networks on CIFAR-10 dataset, from which every $(32\times 32 \times 3)$ input image is converted to a $3072$-dimensional normalized vector.
%each measures the runtime of a matrix product on CPU.
%which are data points of the runtime of matrix products on CPU.
% with $241,600$ samples. It contains data on runtime measurements of a matrix-matrix product $AB = C$, where all matrices have size $(2048 \times 2048)$, using a parameterizable SGEMM GPU kernel with $241,600$ possible parameter combinations. 
% \\
Experiment on the SGEMM dataset are presented in the supplementary material

\begin{wraptable}{r}{0.4\textwidth}
     \caption{MSE for different architectures for CIFAR-$10$}
     \label{tab:experiment}
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
         \textbf{Architecture} & \textbf{ReLU} & \textbf{GRelu} \\ \hline
         \makecell{Depth $6$, \\ Width $10$k} & $0.48$ & $0.02$  \\ \hline
         \makecell{Depth $7$, \\Width $10$k} & $0.27$ & $0.01$  \\ \hline
         \makecell{Depth $4$, \\Width $15$k} & $0.75$ & $0.03$  \\ \hline
    \end{tabular}
\end{wraptable}

We proceed to CIFAR-$10$. This time, we initialize the ReLU network with the initialization suggested by~\citep{allen2019convergence}, that produces initial predictions of smaller absolute value, and corresponding smaller initial loss. We train both networks with a fixed learning rate of $10^{-4}$ and summarize the results in Table~\ref{tab:experiment}.
All variants of GReLU converged to near zero losses. ReLU variants improved with depth, but did not reach similar losses.
Possibly deeper ReLU networks with fine-tuned learning rates would reach near zero losses as well. The losses of the $4$-layer networks from the table are plotted in Figure~\ref{fig:train_loss_cifar}. It can be seen that the GReLU network suffers higher initial loss due to its unique initialization, and converges with a higher rate to its optimum.
In addition, as stated in theorem \ref{thm:equivalence2}, there is an equivalence between GReLU and ReLU networks, that is, for any GReLU network, one can find a counterpart ReLU network such as the outputs of every layer of the two networks correspond. In figure \ref{fig:grelu_relu_cifar}, we show the training and validation loss on CIFAR-10 dataset trained with augmentations both for GReLU and ReLU, when, at epoch 40, the GReLU is transformed into a ReLU network as stated in Theorem (\ref{thm:equivalence2}). One can observe that this transition leads to a better generalization that its ReLU counterpart trained without transformations from GReLU. The transition point in epoch 40 is interesting, since we do not see any difference on the training loss, but the validation loss is reduced significantly, due to the good generalization ability of ReLU networks. 
% ReLU variants
% ReLU variants improved with depth, but did not reach similar results for the 
% while ReLU did not, but possibly a deeper ReLU networks would. 
% Figure~\ref{fig:train_loss_cifar}
% comparison of depth and width by previous works. 
% \\
%  The chosen learning rate is the one that lead to a stable training and does not diverge or oscillate too much. We can see that our method converges faster and is more stable allowing  higher learning rate. While our method can converge with a learning rate of $10^{-3}$, the maximum learning rate that would not lead to divergence for regular Relu is $10^{-4}$. When multiplying this latter by two, we can already see the training loss getting unstable.  In Figure \ref{fig:train_loss_sgemm3}, we present the evolution of the loss when using same learning rate for both regular and Gated ReLU's. We can observe that the Gated ReLU network has a more stable training, meaning a monotone loss decrease, and converges faster to a lower MSE.
% In order to explain the reason for the fact that our method allows a higher learning rate, for every step, we compute the MSE between the gradients of the current and previous step, and present this difference as function of a step in Figure \ref{fig:train_loss_grad} both for our method and regular ReLU when using a stable learning rate for both methods of $10^{-4}$. The higher this difference, the less stable is the training, since it would imply that the gradients change a lot during the training. In Figure \ref{fig:successive_relu_hamming}, we present the mean hamming distance between the activation patterns of the ReLU at two consecutive epochs. For this, we select a subset of input data, and record the pattern of the activated ReLU for the network at epoch $e$ and $e+1$, and compute the average hamming distance between them on all images, layers, and neurons in the network. W can observe that as the training evolves, this activation pattern for ReLU network changes more and more, while it does not vary at all (by definition) for our Gated ReLU, that could explain the fact that the training is more stable, and that the gradients in our network vary less than the ones in the ReLU one. As predicted by Theorem \ref{thm:NTK}, we can observe that, unlike regular ReLU, this difference does not increase along the training and even get smaller, leading to a more stable training and allowing higher learning rates. 
% Finally, we show the impact of the number of channels and layers in Figure \ref{fig:train_loss_sgemm2}. As can be seen, it seems that our method performs better with deeper network than with shallower wider ones.
%We also use the highest possible learning rate that does not lead to divergence. For Gated ReLU; the learning rate is $7\cdot10^{-5}$ while for regular ReLU, the learning rate used is $2\cdot10^{-5}$.  In addition, we also compare the convergence of our network using the same learning rate as the regular ReLU one (even though the latter is not optimal for our metehod). We train the regression for 600 epochs, using SGD with Nesterov momentum set to $0.9$. Figure \ref{fig:train_loss_sgemm} shows the evolution of the MSE as a function of epochs. We can see that using gated Relu leads to faster convergence, but also to a lower MSE, not only using the maximum possible learning rate, but also using a lower learning rate that leads to more stable convergence. The fact that we do not reach zero error is because we do not train the network until full convergence, as the theory shows that this would require a significantly higher number of epochs. In addition, we show the impact of the number of channels and layers in Figure \ref{fig:train_loss_sgemm2}. As can be seen, it seems that our method performs better with deeper network than with shallower wider ones.

  
  
  \begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/train_err_cifar10.pdf}
        \caption{Train MSE w.o. augmentations}
        \label{fig:train_loss_cifar}
    \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
            \includegraphics[width=\textwidth]{figures/graph_train_GReLU_ReLU.pdf}
            \caption{Train MSE vs epoch}
        \label{fig:train_loss_grelu_relu_cifar}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
            \centering
    \includegraphics[width=\textwidth]{figures/graph_test_GReLU_ReLU.pdf}
    \caption{Test MSE vs epoch}
    \label{fig:test_loss_grelu_relu_cifar}
    \end{subfigure}
    \caption{MSE as a function of epochs for CIFAR dataset with (middle and right) and without (left) augmentations for GReLU and ReLU. Two left most graphs show the experiment where the GReLU is transformed into ReLU at epoch 40.}
  \label{fig:grelu_relu_cifar}
\end{figure}
  
  
  
%\end{table}
%\end{figure}


% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.49\textwidth}
%     \includegraphics[width=\textwidth]{figures/theory_graph.pdf}
%     \caption{MSE vs epochs for theoretic and sub-theoretic widths of a $4$-layers network.}
%     \label{fig:theory_graph}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\textwidth}
%     \includegraphics[width=\textwidth]{figures/train_err_cifar10.pdf}
%     \caption{Training loss as a function of epochs for regular and custom ReLU on CIFAR-10}
%     \label{fig:train_loss_cifar}
%   \end{minipage}
% \end{figure}



% \paragraph{CIFAR-10}
% We also implement our method on CIFAR-10 dataset.
% For all of our experiments, we train our networks on CIFAR-10 dataset, from which every $(32\times 32 \times 3)$ input image is converted to a $3072$-dimensional normalized vector. We initialize the FC network as described in Section~\ref{sec:preliminaries}. Every exeriment is conducted with the same hyper parameters. We train both networks with learning rate $10^{-4}$. %Even though the Cifar dataset is a classification dataset, where the conventional loss is computed as a cross entropy between the softmax of the output logits and the true target, in our setting, 
% We express the problem as a regression one and use a mean squared error between the output logits and the one-hot vector encoding the correct class.  Results are presented in the below table:
% \begin{table}[h]
%     \centering
%     \begin{tabular}{|c|c|c|}
%     \hline
%          Architecture & ReLU & GRelu \\ \hline
%          6 layers, 10k neurons & 0.48 & 0.02  \\ \hline
%          7 layers, 10k neurons & 0.27 & 0.01  \\ \hline
%          4 layers, 15k neurons & 0.75 & 0.03  \\ \hline
%     \end{tabular}
%     \caption{CIFAR-$10$ error}%Training error for regular and Gated ReLU's on Cifar 10}
%     \label{tab:experiment}
% \end{table}
% In Figure \ref{fig:train_loss_cifar}, we show the evolution of the training loss as a function of epoch for Gated and Regular ReLU on CIFAR 10 using a FC network with 4 layers and 15k channels. We can see that the training loss of the Gated ReLU network converges to zero much faster that the one with Regular ReLU.
% \begin{wrapfigure}[14]{r}{0.5\textwidth}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/train_err_cifar10.pdf}
%     \caption{Training loss as a function of epochs for regular and custom ReLU on CIFAR-10}
%     \label{fig:train_loss_cifar}
% \end{wrapfigure}
% \asaf{If we put a table (2) instead of graph it can contain: 1. test error (once, so we can focus on train-error in graphs. 2. FLOPS, so no one will miss the ~50 percent improvement :) \\
% Synthetic - better \citep something on the selected function. Also, not sure what is the point behind the current experiment (let's discuss).}
\subsection{Training Dynamics}
To answer \textbf{question 3}, we start with a comparison of the optimization trajectories of the networks. Regular trajectories are favored due to typically smoother corresponding optimization landscapes. Acceleration methods like gradient-descent with momentum~\citep{qian1999momentum} provide more regular trajectories and are commonly used. During a full train with each network with $\eta=10^{-4}$, we compute the $\ell_2$ norm between consecutive gradients, $\|g_t-g_{t-1}\|_2$, and present the results in Figure~\ref{fig:train_loss_grad}. The gradient differences of the GReLU network are smaller than the ones of the ReLU network, and
gradually decrease along the convergence to the global optima.
This provides an additional empirical validation of the relatively larger learning rates allowed by our theory. In addition, this empirical evaluation matches the tighter bound on the gradients difference guaranteed by theorem~\ref{thm:NTK}. The gradient differences of the ReLU network increase monotonically along the training, with highly irregular trajectories that match the relatively high variation of the losses in Figure~\ref{fig:train_loss_sgemm3}.
\\
To better understand the behaviour of the ReLU network, we conduct an additional experiment, of calculating the change in its activation patterns along the training. More specifically, we present the mean Hamming distance between its activation patterns at consecutive epochs. The distance is computed across all ReLU activations over a selected validation set.
The results are illustrated in Figure~\ref{fig:successive_relu_hamming} and are quite surprising: a large portion of the activations, $20\%-25\%$, changes every epoch and keep increasing along the run. This result complements the previous one by showing some instability of the ReLU network. 
% In an additional experiment, in order to better understand the behaviour of the ReLU network, we also plot the change in its activation patterns along the training in Figure~\ref{fig:successive_relu_hamming}. 
% More specifically we present the mean hamming distance between its activation patterns at consecutive epochs. We compute the distance across all $mL$ ReLU activations over a selected validation set. 
% The results are quite surprising, a large portion of the activations, $20\%-25\%$, changes every epoch and keep increasing along the run. This result complements the previous one by showing some instability of the ReLU network. 
% We point out that such instability could possibly offer an implicit regularization in exchange and proves useful, and some hybrid version of the GReLU network, that allows smaller, controlled changes in its activation patterns is an interesting future direction.
We point out that some level of change in activation patterns along the optimization possibly contributes to the generalization via implicit regularization.
In such case, a hybrid version of the GReLU network that allows gradual, controlled changes of its activation patterns is an interesting future direction to be pursued.




==> extensions.tex <==
\section{extensions}
TODO:
\begin{itemize}
    \item Replace $O()$ with precise constants. 
    \item related - 2nd half of 2020.
    \item cross-entropy for multi-label - easy, see p40 in Allen's.
    \item SGD
\end{itemize}


Possible extensions:
\begin{itemize}
    \item Convolutional 
    \item residual connections
    \item cross-entropy for multi-label - easy, see p40 in Allen's.
    \item SGD
\end{itemize}
Will run experiments mostly with the above.


==> heavy_ball.tex <==
\section{Convergency Analysis for the Heavy Ball Method}

According to the updating rule of the heavy ball method, we have
\[
    W_{t+1,k} = W_{t,k} - \eta \nabla_k \ell(W_t) + \nu \left(W_{t,k} - W_{t-1, k}\right)
\]
We can thus write $W^i_{t+1} - W^i_t$ as
\begin{eqnarray*}
\lefteqn{W^i_{t+1} - W^i_t} \\
& = & B\left(\prod_{k=1}^L D_k^i\left(W_{t,k} - \eta \nabla_k \ell(W_t) + \nu\left(W_{t,k} - W_{t-1,k}\right)\right)\right)C - B\left(\prod_{k=1}^L D_k^i W_{t,k}\right)C \\
& = & -\eta\sum_{k=1}^L F_{t,k+1}^i \nabla_k\ell(W_t) G_{t,k+1}^i + \nu\sum_{k=1}^L F_{t,k+1}^i\left(W_{t,k} - W_{t-1,k}\right)G_{t,k-1}^i \\
&   & + \sum_{s=2}^L \sum_{k_1>\ldots>k_s}F_{t,k_1+1}^iD_{k_1}^i\left(W_{t+1,k_1} - W_{t,k_1}\right)\left(\prod_{a=1}^{s-1} Z_{t, k_a+1: k_{a+1}}^i\left(W_{t+1,k_{a+1}} - W_{t,k_{a+1}}\right)\right)G_{t, k_s-1}^i \\
& = & -\eta\sum_{k=1}^L F_{t,k+1}^i \left[F_{t,k+1}^i\right]^{\top}\left(W^i_{t} - \Phi_i\right)x_ix_i^{\top}\left[G_{t,k-1}^i\right]^{\top}G_{t,k-1}^i + \nu\sum_{k=1}^L F_{t,k+1}^i\left(W_{t,k} - W_{t-1,k}\right)G_{t,k-1}^i \\
&   & - \eta\sum_{k=1}^L \sum_{j \neq i} F_{t,k+1}^i \left[F_{t,k+1}^j\right]^{\top}\left(W^j_{t+1} - \Phi_j\right)x_jx_j^{\top}\left[G_{t,k-1}^j\right]^{\top}G_{t,k-1}^i \\
&   & + \underbrace{\sum_{s=2}^L \sum_{k_1>\ldots>k_s}F_{t,k_1+1}^iD_{k_1}^i\left(W_{t+1,k_1} - W_{t,k_1}\right)\left(\prod_{a=1}^{s-1} Z_{t, k_a+1: k_{a+1}}^i\left(W_{t+1,k_{a+1}} - W_{t,k_{a+1}}\right)\right)G_{t, k_s-1}^i}_{:= \Delta_{t,i}}
\end{eqnarray*}
where
\[
    Z^i_{t,k_a:k_b} = \left(\prod_{k=k_a}^{k_b} D_{k}^i W_{t,k}\right)D_{k_b}^i
\]
Following the same analysis as before, we have
\begin{eqnarray*}
\ell(W_{t+1}) - \ell(W_t) = \sum_{i=1}^n \left\langle \left(W_{t+1}^i - W^i_t\right)x_i, \left(W_t^i - \Phi_i\right)x_i\right\rangle + \frac{1}{2}\left|\left(W_{t+1}^i - W_t^i\right)x_i\right|^2
\end{eqnarray*}
We will bound the first and second terms separately.


We first deal with $\sum_{i=1}^n \langle W_{t+1}^i - W^i_t, W_t^i - \Phi_i\rangle$, i.e.
\begin{eqnarray*}
\lefteqn{\sum_{i=1}^n\left\langle \left(W_{t+1}^i - W^i_t\right)x_i, \left(W_t^i - \Phi_i\right)x_i\right\rangle} \\
& = & -\eta\sum_{i=1}^n\sum_{k=1}^L \left|\left\langle \left[F_{t,k+1}^i\right]^{\top}\left(W^i_{t} - \Phi_i\right)x_ix_i^{\top}\left[G_{t,k-1}^i\right]^{\top}\right\rangle\right|^2 \\
&   & + \nu\sum_{i=1}^n\sum_{k=1}^L \left\langle W_{t,k} - W_{t-1,k}, \left[F_{t,k+1}^i\right]^{\top}\left(W_t^i - \Phi_i\right)x_ix_i^{\top}\left[G_{t,k-1}^i\right]^{\top}\right\rangle \\
&   & - \eta\sum_{i=1}^n\sum_{k=1}^L \sum_{j \neq i} \left\langle F_{t,k+1}^i \left[F_{t,k+1}^j\right]^{\top}\left(W^j_{t+1} - \Phi_j\right)x_jx_j^{\top}\left[G_{t,k-1}^j\right]^{\top}G_{t,k-1}^i, \left(W_t^i - \Phi_i\right)x_ix_i^{\top}\right\rangle \\
&   & + \sum_{i=1}^n\left\langle\Delta_{t,i}, (W_t^i - \Phi_i)x_ix_i^{\top}\right\rangle
\end{eqnarray*}
Define
\[
\Omega_{t}^i = W_t^i - W_{t-1}^i - \sum_{k=1}^L F_{t,k+1}^i\left(W_{t,k}^i - W_{t-1,k}^i\right)G_{t,k-1}^i
\]
We have
\begin{eqnarray*}
\lefteqn{\sum_{i=1}^n\left\langle \left(W_{t+1}^i - W^i_t\right)x_i, \left(W_t^i - \Phi_i\right)x_i\right\rangle} \\
& = & -\eta\sum_{i=1}^n\sum_{k=1}^L \left|\left\langle \left[F_{t,k+1}^i\right]^{\top}\left(W^i_{t} - \Phi_i\right)x_ix_i^{\top}\left[G_{t,k-1}^i\right]^{\top}\right\rangle\right|^2 \\
&   & + \nu\sum_{i=1}^n \left\langle W_t^i - W_{t-1}^i, (W_t^i - \Phi_i)x_ix_i^{\top} \right\rangle + \nu \sum_{i=1}^n \left\langle \Omega_t^i, (W_t^i - \Phi_i)x_ix_i^{\top} \right\rangle  \\
&   & - \eta\sum_{i=1}^n\sum_{k=1}^L \sum_{j \neq i} \left\langle F_{t,k+1}^i \left[F_{t,k+1}^j\right]^{\top}\left(W^j_{t+1} - \Phi_j\right)x_jx_j^{\top}\left[G_{t,k-1}^j\right]^{\top}G_{t,k-1}^i, \left(W_t^i - \Phi_i\right)x_ix_i^{\top}\right\rangle \\
&   & + \sum_{i=1}^n \left\langle\Delta_{t,i}, (W_t^i - \Phi_i)x_ix_i^{\top}\right\rangle \\
& \leq & -2\eta L\left(\alpha^2 - n\gamma\beta^2\right)\ell(W_t) + \nu\left(\ell(W_t) - \ell(W_{t-1}) + \frac{1}{2}|W_t^i - W_{t-1}^i|^2\right) \\
&      & + \sum_{i=1}^n \left\langle \Delta_{t,i}x_i, \left(W_t^i - \Phi_i\right)x_i\right\rangle + \nu \sum_{i=1}^n \left\langle \Omega_t^i, \left(W_t^i - \Phi_i\right)x_ix_i^{\top} \right\rangle
\end{eqnarray*}
Define
\[
\rho_{\Delta} = \sum_{i=1}^n \left|\Delta_t^i\right|^2, \quad \rho_{\Omega} = \sum_{i=1}^n \left|\Omega_t^i\right|^2
\]
We have
\begin{eqnarray*}
\lefteqn{\sum_{i=1}^n\left\langle \left(W_{t+1}^i - W^i_t\right)x_i, \left(W_t^i - \Phi_i\right)x_i\right\rangle} \\
& \leq & -\left(\eta L\left(\alpha^2 - 2n\gamma\beta^2\right) - \nu\right)\ell(W_t) - \nu \ell(W_{t-1}) + \frac{\nu}{2} \sum_{i=1}^n |W_t^i - W_{t-1}^i|^2 + \frac{1}{\eta\alpha^2 L}\left(\rho_{\Delta} + \nu^2 \rho_{\Omega}\right)
\end{eqnarray*}

We are now dealing with $|W^i_{t+1} - W^i_t|^2$.
\begin{eqnarray*}
\lefteqn{\sum_{i=1}^n\left|W^i_{t+1} - W^i_t\right|^2} \\
& \leq & 4\sum_{i=1}^n\left|-\eta\sum_{k=1}^L F_{t,k+1}^i \left[F_{t,k+1}^i\right]^{\top}\left(W^i_{t} - \Phi_i\right)x_ix_i^{\top}\left[G_{t,k-1}^i\right]G_{t,k-1}^i + \nu\left(W_t^i - W_{t-1}^i\right)\right|^2 + 4\nu^2\rho_{\Omega}\\
&   & + 4\eta^2\sum_{i=1}^n \left|\sum_{k=1}^L \sum_{j \neq i} F_{t,k+1}^i \left[F_{t,k+1}^j\right]^{\top}\left(W^j_{t+1} - \Phi_j\right)x_jx_j^{\top}\left[G_{t,k-1}^j\right]^{\top}G_{t,k-1}^i\right|^2 + 4\rho_{\Delta} \\
& \leq &4\eta^2\sum_{i=1}^n\left|\sum_{k=1}^L F_{t,k+1}^i \left[F_{t,k+1}^i\right]^{\top}\left(W^i_{t} - \Phi_i\right)x_ix_i^{\top}\left[G_{t,k-1}^i\right]G_{t,k-1}^i\right|^2 + 4\nu^2\sum_{i=1}^n |W_t^i - W_{t-1}^i|^2 + 4\nu^2\rho_{\Omega} \\
&      &-8\eta\nu\sum_{i=1}^n\sum_{k=1}^L \left\langle F_{t,k+1}^i\left[F_{t,k+1}^i\right]^{\top}\left(W_t^i - \Phi_i\right)\left[G^i_{t,k-1}\right]^{\top}G^i_{t,k-1}, W_t^i - W_{t-1}^i \right\rangle \\
&      & + 4\eta^2\sum_{i=1}^n \left|\sum_{k=1}^L \sum_{j \neq i} F_{t,k+1}^i \left[F_{t,k+1}^j\right]^{\top}\left(W^j_{t+1} - \Phi_j\right)x_jx_j^{\top}\left[G_{t,k-1}^j\right]^{\top}G_{t,k-1}^i\right|^2 + 4\rho_{\Delta} \\
& \leq & 8\eta^2\beta^4L^2\ell(W_t) + 4\nu^2\sum_{i=1}^n|W^i_t - W^i_{t-1}|^2 + 4\nu^2\rho_{\Omega}\\
&      & + 8\eta\nu L\alpha^2\left(\ell(W_{t-1}) - \ell(W_t) - \frac{1}{2}\sum_{i=1}^n |W_t^i - W_{t-1}^i|^2\right) \\
&    & + 4\eta\nu\left(2\epsilon + \epsilon^2\right)\alpha^2L\sum_{i=1}^n \left(|W_t^i - \Phi_i|^2 + |W_t^i - W_{t-1}^i|^2\right)\\
&      & + 8\eta^2L^2n^2\gamma^2\beta^4\ell(W_t) + 4\rho_{\Delta} \\
& \leq & \left(8\eta^2\beta^4L^2(1 + \gamma^2n^2) + 8(2\epsilon + \epsilon^2)\nu\alpha^2\eta L - 8\nu\alpha^2\eta L\right)\ell(W_t) + 8\nu\alpha^2\eta L\ell(W_{t-1})\\
&      & + 4\nu\left(\nu - \left(1 - 2\epsilon - \epsilon^2)\right)\alpha^2\eta L\right)\sum_{i=1}^n |W_t^i - W^i_{t-1}|^2 \\
&      & + 4\nu^2\rho_{\Omega} + 4\rho_{\Delta}
\end{eqnarray*}
By putting the above two inequalities together, we have
\begin{eqnarray*}
\lefteqn{\ell(W_{t+1}) - \ell(W_t)} \\
& \leq & \left(\underbrace{8\eta^2\beta^4L^2(1 + \gamma^2n^2) + 8(2\epsilon + \epsilon^2)\nu\alpha^2\eta L + 2n\gamma\beta^2\eta L}_{:=\varphi} -\alpha^2\eta L + \nu - 8\nu\alpha^2\eta L\right)\ell(W_t) + (8\nu\alpha^2\eta L - \nu)\ell(W_{t-1})\\
&      & + 4\nu\left(\nu - \left(1 - 2\epsilon - \epsilon^2)\right)\alpha^2\eta L + \frac{1}{8}\right)\sum_{i=1}^n |W_t^i - W^i_{t-1}|^2 + \left(4\nu^2\rho_{\Omega} + 4\rho_{\Delta}\right)\left(1 + \frac{1}{\alpha^2\eta L}\right)
\end{eqnarray*}

Since with a probability $1 - 3\sqrt{m}L^2\exp(-\Omega(m/L))$,
\[
\left|F_{t,k_1+1}^iD_{k_1}^i\left(W_{t+1,k_1} - W_{t,k_1}\right)\left(\prod_{a=1}^{s-1} Z_{t, k_a+1: k_{a+1}}^i\left(W_{t+1,k_{a+1}} - W_{t,k_{a+1}}\right)\right)G_{t, k_s-1}^ix_i\right| \leq \beta^{(s+1)/2}|W_{t+1} - W_t|^s_2
\]
we have
\[
\left|\Delta_{t,i}x_i\right|^2 \leq \left(\sum_{s=2}^L L^s\beta^{(s+1)/2}\left|W_{t+1} - W_t\right|^s_2\right)^2 \leq \frac{L^4\beta^{3}\tau^2}{\left(1 - L\sqrt{\beta}\tau\right)^2}|W_{t+1} - W_t|^2 \leq 2L^4\beta^{3}\tau^2|W_{t+1} - W_t|^2
\]
and therefore
\[
\rho_{\Delta} \leq \underbrace{2nL^4\beta^{3}\tau^2}_{:=\xi}|W_{t+1} - W_t|^2 \leq \xi|W_{t+1} - W_t|^2
\]
Similarly, we have
\[
\rho_{\Omega} \leq 2nL^4\beta^{3}\tau^2|W_{t} - W_{t-1}|^2 \leq \xi |W_t - W_{t-1}|^2
\]
As a result, we have
\begin{eqnarray*}
\lefteqn{\ell(W_{t+1}) - \ell(W_t)} \\
& \leq & \left(\varphi  -\alpha^2\eta L + \nu - 8\nu\alpha^2\eta L\right)\ell(W_t) + (8\nu\alpha^2\eta L - \nu)\ell(W_{t-1})\\
&      & + 4\nu\left(\nu - \left(1 - 2\epsilon - \epsilon^2)\right)\alpha^2\eta L + \frac{1}{8}\right)\sum_{i=1}^n |W_t^i - W^i_{t-1}|^2 \\
&      & + \underbrace{4\xi\left(1 + \frac{1}{\alpha^2\eta L}\right)}_{:=\pi}\left(|W_{t+1} - W_t|^2 + \nu^2|W_t - W_{t-1}|^2 \right) \\
& \leq & \left(\varphi  -\alpha^2\eta L - \nu - 8\nu\alpha^2\eta L\right)\ell(W_t) + (8\nu\alpha^2\eta - \nu) L\ell(W_{t-1}) \\
&      & + \left(4\nu^2+2\nu\right)\sum_{i=1}^n |W_t^i - W^i_{t-1}|^2 + \pi\left(|W_{t+1} - W_t|^2 + \nu^2|W_t - W_{t-1}|^2 \right)
\end{eqnarray*}
Consider $\ell(W_{t+1}) - \ell(W_t) + a\sum_{i=1}^n |W_{t+1}^i - W_t^i|^2 + b|W_{t+1} - W_t|^2$. We have
\begin{eqnarray*}
\lefteqn{\ell(W_{t+1}) - \ell(W_t) + a\sum_{i=1}^n |W_{t+1}^i - W_t^i|^2 + b|W_{t+1} - W_t|^2} \\
& \leq & \left((a+1)\varphi  -\alpha^2\eta L + \nu - 8(a+1)\nu\alpha^2\eta L\right)\ell(W_t) + (8(a+1)\nu\alpha^2\eta L - \nu) \ell(W_{t-1}) \\
&      & + \left(4(a+1)\nu^2+2\nu\right)\sum_{i=1}^n |W_t^i - W^i_{t-1}|^2 + \pi(a+1)\left(|W_{t+1} - W_t|^2 + \nu^2|W_t - W_{t-1}|^2 \right)
\end{eqnarray*}
and therefore
\begin{eqnarray*}
\lefteqn{\ell(W_{t+1}) - \ell(W_t) + a\sum_{i=1}^n |W_{t+1}^i - W_t^i|^2 + (b - (a+1)\pi)|W_{t+1} - W_t|^2} \\
& \leq & \left((a+1)\varphi  -\alpha^2\eta L + \nu - 8(a+1)\nu\alpha^2\eta L\right)\ell(W_t) + (8(a+1)\nu\alpha^2\eta L - \nu)\ell(W_{t-1}) \\
&      & + \left(4(a+1)\nu^2+2\nu\right)\sum_{i=1}^n |W_t^i - W^i_{t-1}|^2 + \pi(a+1)\nu^2|W_t - W_{t-1}|^2 + b|W_{t+1} - W_t|^2
\end{eqnarray*}
Assume $a \geq 1$, 
Since
\begin{eqnarray*}
\lefteqn{\left|W_{t+1} - W_t\right|^2} \\
& \leq & \nu^2\sum_{k=1}^L |W_{t,k} - W_{t,k-1}|^2 + \eta^2\sum_{k=1}^L \left|\nabla_k \ell(W_t)\right|^2 \\
&      & -2\eta\nu\sum_{i=1}^n \sum_{k=1}^L \left\langle\left[F^i_{t,k+1}\right]^{\top}\left(W^i_t - \Phi_i\right)x_ix_i^{\top}\left[G_{t,k-1}^i\right]^{\top}, W_{t,k} - W_{t,k-1} \right\rangle\\
& \leq & \nu^2|W_t - W_{t-1}|^2 + 2\eta^2L\beta^2 \ell(W_t) - 2\eta\nu\sum_{i=1}^n \left\langle (W^i_t - \Phi_i)x_ix_i^{\top}, W^i_{t} - W^i_{t-1} \right\rangle + 2\eta\nu\sum_{i=1}^n \left|W^i_t - \Phi_i\right|\left|\Omega_t^i\right| \\
& \leq & \nu^2|W_t - W_{t-1}|^2 - 2\eta\left(\nu(1-\frac{\alpha^2 L}{4b\nu}) - \eta \beta^2 L\right)\ell(W_t) + 2\eta\nu\ell(W_{t-1})\\
&      & - \eta\nu\sum_{i=1}^n |W_t^i - W_{t-1}^i|^2 + \frac{4b\eta\nu\xi}{\alpha^2 L }|W_t - W_{t-1}|^2
\end{eqnarray*}
we have
\begin{eqnarray*}
\lefteqn{\ell(W_{t+1}) - \ell(W_t) + a\sum_{i=1}^n |W_{t+1}^i - W_t^i|^2 + (b - (a+1)\pi)|W_{t+1} - W_t|^2} \\
& \leq & \left((a+1)\varphi + 2b\eta^2\beta^2 L  -\frac{\alpha^2\eta L}{2} -2b\eta\nu + \nu - 8(a+1)\nu\alpha^2\eta L\right)\ell(W_t) + (8(a+1)\nu\alpha^2\eta - \nu + 2b\eta\nu) L\ell(W_{t-1}) \\
&      & + \left(4(a+1)\nu^2+2\nu-b\eta\nu\right)\sum_{i=1}^n |W_t^i - W^i_{t-1}|^2 + \left(b + \pi(a+1) + \pi b^2\eta\nu\right)\nu^2|W_t - W_{t-1}|^2 \\
& \leq & \left(-\frac{\alpha^2\eta L}{4} - 2b\eta\nu + \nu - 8(a+1)\nu\alpha^2\eta L\right)\ell(W_t) + (8(a+1)\nu\alpha^2\eta - \nu + 2b\eta\nu) L\ell(W_{t-1}) \\
&      & + (a+1)\left(4\nu^2+2\nu\right)\sum_{i=1}^n |W_t^i - W^i_{t-1}|^2 + \left(b + \pi(a+1) + \pi b^2\eta\nu\right)\nu^2|W_t - W_{t-1}|^2
\end{eqnarray*}
Since $\pi$ is a very small number, we could safely assume that $b \geq 2\pi(a+1) + 2\pi b^2\eta\nu$, we thus have
\begin{eqnarray*}
\lefteqn{\ell(W_{t+1}) - \ell(W_t) + a\sum_{i=1}^n |W_{t+1}^i - W_t^i|^2 + \frac{b}{2}|W_{t+1} - W_t|^2} \\
& \leq & \left(-\frac{\alpha^2\eta L}{4} - 2b\eta\nu + \nu - 8(a+1)\nu\alpha^2\eta L\right)\ell(W_t) + (8(a+1)\nu\alpha^2\eta L- \nu + 2b\eta\nu) \ell(W_{t-1}) \\
&      & + (a+1)\left(4\nu^2+2\nu\right)\sum_{i=1}^n |W_t^i - W^i_{t-1}|^2 + \frac{3\nu^2}{2}b|W_t - W_{t-1}|^2 \\
& \leq & \left(-\frac{\alpha^2\eta L}{4} - 2b\eta\nu + \nu - 8(a+1)\nu\alpha^2\eta L\right)\ell(W_t) + (8(a+1)\nu\alpha^2\eta L - \nu + 2b\eta\nu) \ell(W_{t-1}) \\
&      & + \frac{a+1}{a}\left(4\nu^2+2\nu\right)\left(a\sum_{i=1}^n |W_t^i - W^i_{t-1}|^2 + \frac{b}{2}|W_t - W_{t-1}|^2\right)
\end{eqnarray*}
Hence, according to Lemma 1 from ``Global convergence of the Heavy-ball method for convex optimization'', we have
\[
    \ell(W_{t+1}) \leq 2(1 - q)^t\ell(W_1)
\]
where
\[
q \leq \max\left(\frac{a+1}{a}\left(4\nu^2 + 2\nu\right), 1 - \frac{\alpha\sqrt{\eta L}}{4}\right)
\]
By choosing small enough $\nu$, we will have
\[
    q \leq 1 - \frac{\alpha\sqrt{\eta L}}{4}
\]

\end{document}


and
\[
\left|W^i_{t,k} - W^i_{t,k-1} - \sum_{k=1}^L F_{t,k+1}^i\left(W_{t,k} - W_{t-1, k}\right)G_{t,k-1}^i\right| \leq \frac{L\beta\tau}{1 - L\beta\tau} |W_t - W_{t-1}| \leq 2L\beta\tau|W_t - W_{t-1}|
\]
we have
\[
|W_{t+1} - W_t|^2 \leq \left(\nu^2 + 4\eta\nu\beta^2\tau \right)|W_t - W_{t-1}|^2 - 2\eta\left(\nu - \eta \beta^2 L\right)\ell(W_t) + 4\eta\nu\ell(W_{t-1})
\]



Since
\begin{eqnarray*}
\lefteqn{-\left\langle F_{t,k+1}^i\left[F_{t,k+1}^i\right]^{\top}\left(W_t^i - \Phi_i\right)\left[G_{t,k-1}^i\right]^{\top}G_{t,k-1}^i, \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i \right\rangle} \\
& \leq & -\alpha^2\left\langle W_t^i - \Phi_i,  \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i \right\rangle + \epsilon\alpha^2\sum_{k'=1}^L |W_t^i - \Phi_i|\left|F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i\right|\\
& \leq & -\alpha^2\left\langle W_t^i - \Phi_i,  \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i \right\rangle + \frac{\epsilon\alpha^2L}{2}|W_t^i - \Phi_i|^2 + \frac{\epsilon\alpha^2\beta^2L}{2}\left|W_{t} - W_{t-1}\right|^2 \\
& \leq & -\alpha^2\left\langle W_t^i - \Phi_i,  W^i_t - W^i_{t-1} \right\rangle + \frac{\epsilon\alpha^2L}{2}|W_t^i - \Phi_i|^2 + \frac{\epsilon\alpha^2\beta^2L}{2}\left|W_{t} - W_{t-1}\right|^2 \\
&      & + \alpha^2|W_t^i - \Phi_i|\left|W^i_t - W^i_{t-1} - \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i\right| \\
& \leq & \alpha^2\left(\frac{1}{2}|W_{t-1}^i - \Phi_i|^2 - \frac{1}{2}|W_{t}^i - \Phi_i|^2 - \frac{1}{2}|W_t^i - W_{t-1}^i|^2\right)+ \frac{\epsilon\alpha^2L}{2}|W_t^i - \Phi_i|^2 + \frac{\epsilon\alpha^2\beta^2L}{2}\left|W_{t} - W_{t-1}\right|^2 \\
&      & + \alpha^2|W_t^i - \Phi_i|\left|W^i_t - W^i_{t-1} - \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i\right|
\end{eqnarray*}
we have
\begin{eqnarray*}
\lefteqn{\sum_{i=1}^n \sum_{k=1}^L\left\langle F_{t,k+1}^i\left[F_{t,k+1}^i\right]^{\top}\left(W_t^i - \Phi_i\right)\left[G_{t,k-1}^i\right]^{\top}G_{t,k-1}^i, \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i \right\rangle} \\
& \leq & \frac{\alpha^2 L}{2}\ell(W_{t-1}) - \frac{\alpha^2L(1 - 2\epsilon L)}{2}\ell(W_t) + \frac{\epsilon n \alpha^2 \beta^2 L^2}{2}|W_t - W_{t-1}|^2 \\
&      & + \frac{n\alpha^2}{2\epsilon}\left|W^i_t - W^i_{t-1} - \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i\right|^2
\end{eqnarray*}
Since
\[
\left|W^i_t - W^i_{t-1} - \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i\right| \leq \frac{L\tau\beta|W_t - W_{t-1}|}{1 - L\tau\beta} \leq 2L\beta\tau|W_t - W_{t-1}|
\]
we have
\begin{eqnarray*}
\lefteqn{\sum_{i=1}^n \sum_{k=1}^L\left\langle F_{t,k+1}^i\left[F_{t,k+1}^i\right]^{\top}\left(W_t^i - \Phi_i\right)\left[G_{t,k-1}^i\right]^{\top}G_{t,k-1}^i, \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i \right\rangle} \\
& \leq & \frac{\alpha^2 L}{2}\ell(W_{t-1}) - \frac{\alpha^2L(1 - 2\epsilon L)}{2}\ell(W_t) + n\alpha^2\beta^2 L^2\left(\frac{\epsilon}{2}+\frac{\tau^2}{\epsilon}\right)|W_t - W_{t-1}|^2 \\
& \leq & \frac{\alpha^2 L}{2}\ell(W_{t-1}) - \frac{\alpha^2L(1 - 2\epsilon L)}{2}\ell(W_t) + n\alpha^2\beta^2\epsilon|W_t - W_{t-1}|^2
\end{eqnarray*}
and therefore
\begin{eqnarray*}
\lefteqn{\sum_{i=1}^n |W_{t+1}^i - W_t^i|^2} \\
& \leq & -\left(3\eta\nu\alpha^2 L(1 - 2\epsilon L) -7\eta^2\beta^4L^2\right)\ell(W_t) + 3\eta\nu\alpha^2L\ell(W_{t-1}) + \left(4n\nu^2\beta^2 + n\eta\nu\alpha^2\beta^2\epsilon\right)|W_t - W_{t-1}|^2 \\
& \leq & - 3\eta\nu\alpha^2 L (1 - 3\epsilon L)\ell(W_t) + 3\eta\nu\alpha^2L\ell(W_{t-1}) + 8n\nu^2\beta^2|W_t - W_{t-1}|^2
\end{eqnarray*}
Finally, we have
\begin{eqnarray*}
\lefteqn{\ell(W_{t+1}) - \ell(W_t) \leq  \left(4n\nu^2\beta^2 + \frac{n\nu}{\eta}\right)|W_t - W_{t-1}|^2 } \\
&  & - \left(\frac{3}{2}\eta\nu\alpha^2 L (1 - 3\epsilon L)  - \frac{\eta\alpha^2 L}{2} + 3n\eta\gamma\beta^2L\right) \ell(W_t) + \left(\frac{3}{2}\eta\nu\alpha^2L+n\eta\gamma\beta^2L\right)\ell(W_{t-1})
\end{eqnarray*}
Using the inequality
\[
|W_{t+1} - W_t|^2 \leq \left(\nu^2 + 4\eta\nu\beta^2\tau \right)|W_t - W_{t-1}|^2 - 2\eta\left(\nu - \eta \beta^2 L\right)\ell(W_t) + 4\eta\nu\ell(W_{t-1})
\]
we have
\begin{eqnarray*}
\lefteqn{\ell(W_{t+1}) + \underbrace{\theta\left(4n\nu^2\beta^2 + \frac{n\nu}{\eta}\right)}_{:=b}|W_{t+1} - W_{t}|^2 } \\
& \leq & \underbrace{\left(4n\nu^2\beta^2 + \frac{n\nu}{\eta}\right)\left(1 + \theta\left(\nu^2 + 4\eta\nu\beta^2\tau \right)\right)}_{:=c}|W_t - W_{t-1}|^2 \\
&  & + \underbrace{\left\{1 - \left(\frac{3}{2}\eta\nu\alpha^2 L (1 - 3\epsilon L)  - \frac{\eta\alpha^2 L}{2} + 3n\eta\gamma\beta^2L - 2\theta\eta\left(4n\nu^2\beta^2 + \frac{n\nu}{\eta}\right)\left(\nu - \eta \beta^2 L\right)\right)\right\}}_{:=a_1} \ell(W_t) \\
&  & + \underbrace{\left(\frac{3}{2}\eta\nu\alpha^2L+n\eta\gamma\beta^2L+4\theta\eta\nu\left(4n\nu^2\beta^2 + \frac{n\nu}{\eta}\right)\right)}_{:=a_2}\ell(W_{t-1})
\end{eqnarray*}


Since with a probability $1 - 3\sqrt{m}L^2\exp(-\Omega(m/L))$,
\[
\left|F_{t,k_1+1}^iD_{k_1}^i\left(W_{t+1,k_1} - W_{t,k_1}\right)\left(\prod_{a=1}^{s-1} Z_{t, k_a+1: k_{a+1}}^i\left(W_{t+1,k_{a+1}} - W_{t,k_{a+1}}\right)\right)G_{t, k_s-1}^ix_i\right| \leq \beta^{(s+1)/2}|W_{t+1} - W_t|^s_2
\]
we have
\[
\left|\Delta_{t,i}x_i\right|^2 \leq \left(\sum_{s=2}^L L^s\beta^{(s+1)/2}\left|W_{t+1} - W_t\right|^s_2\right)^2 \leq \frac{L^4\beta^{3}\tau^2}{\left(1 - L\sqrt{\beta}\tau\right)^2}|W_{t+1} - W_t|^2
\]
Since
\begin{eqnarray*}
\lefteqn{\left|W_{t+1} - W_t\right|^2} \\
& \leq & \nu^2\sum_{k=1}^L |W_{t,k} - W_{t,k-1}|^2 + \eta^2\sum_{k=1}^L \left|\nabla_k \ell(W_t)\right|^2 \\
&      & -2\eta\nu\sum_{i=1}^n \sum_{k=1}^L \left\langle\left[F^i_{t,k+1}\right]^{\top}\left(W^i_t - \Phi_i\right)x_ix_i^{\top}\left[G_{t,k-1}^i\right]^{\top}, W_{t,k} - W_{t,k-1} \right\rangle\\
& \leq & \nu^2|W_t - W_{t-1}|^2 + 2\eta^2L\beta^2 \ell(W_t) - 2\eta\nu\sum_{i=1}^n \left\langle W^i_t - \Phi_i, W^i_{t} - W^i_{t-1} \right\rangle \\
&      & + 2\eta\nu\sum_{i=1}^n \left|W^i_t - \Phi_i\right|\left|W^i_{t,k} - W^i_{t,k-1} - \sum_{k=1}^L F_{t,k+1}^i\left(W_{t,k} - W_{t-1, k}\right)G_{t,k-1}^i\right| \\
& \leq & \nu^2|W_t - W_{t-1}|^2 - 2\eta\left(\nu - \eta \beta^2 L\right)\ell(W_t) + 4\eta\nu\ell(W_{t-1}) \\
&      & + \eta\nu\sum_{i=1}^n \left|W^i_{t,k} - W^i_{t,k-1} - \sum_{k=1}^L F_{t,k+1}^i\left(W_{t,k} - W_{t-1, k}\right)G_{t,k-1}^i\right|^2
\end{eqnarray*}
and
\[
\left|W^i_{t,k} - W^i_{t,k-1} - \sum_{k=1}^L F_{t,k+1}^i\left(W_{t,k} - W_{t-1, k}\right)G_{t,k-1}^i\right| \leq \frac{L\beta\tau}{1 - L\beta\tau} |W_t - W_{t-1}| \leq 2L\beta\tau|W_t - W_{t-1}|
\]
we have
\[
|W_{t+1} - W_t|^2 \leq \left(\nu^2 + 4\eta\nu\beta^2\tau \right)|W_t - W_{t-1}|^2 - 2\eta\left(\nu - \eta \beta^2 L\right)\ell(W_t) + 4\eta\nu\ell(W_{t-1})
\]
and therefore
\begin{eqnarray*}
\lefteqn{|\Delta_{t,i}x_i|^2} \\
& \leq & \frac{L^4\beta^{3}\tau^2}{\left(1 - L\sqrt{\beta}\tau\right)^2}\left\{\left(\nu^2 + 4\eta\nu\beta^2\tau \right)|W_t - W_{t-1}|^2 - 2\eta\left(\nu - \eta \beta^2 L\right)\ell(W_t) + 4\eta\nu\ell(W_{t-1})\right\} \\
& \leq & 2\nu^2\beta^3\tau^2 L^4|W_t - W_{t-1}|^2 - 3\eta\beta^3\tau^2L^4\left(\nu - \eta\beta^2L\right)\ell(W_t) + 6\eta\nu\beta^3\tau^2 L^4\ell(W_{t-1}) \\
& \leq & 2\nu^2\beta^3\tau^2 L^4|W_t - W_{t-1}|^2 - \eta\nu\beta^3\tau^2L^4\ell(W_t) + 6\eta\nu\beta^3\tau^2 L^4\ell(W_{t-1})
\end{eqnarray*}
and therefore
\begin{eqnarray*}
\lefteqn{\sum_{i=1}^n\left\langle \left(W_{t+1}^i - W^i_t\right)x_i, \left(W_t^i - \Phi_i\right)x_i\right\rangle} \\
& \leq & -\eta L\left(\frac{\alpha^2}{2} - 2n\gamma\beta^2 - \frac{n\nu\beta^3\tau^2L^2}{\eta\alpha^2}\right)\ell(W_t) + \frac{n\nu}{2\eta}\left(1 + \frac{2\nu\beta^3\tau^2L^3}{\alpha^2}\right)|W_t - W_{t-1}|^2 + \frac{6\nu\beta^3\tau^2 L^3}{\alpha^2}\ell(W_{t-1})\\
& \leq & -\eta L\left(\frac{\alpha^2}{2} - 3n\gamma\beta^2\right)\ell(W_t) + \frac{n\nu}{\eta}|W_t - W_{t-1}|^2 + n\eta\gamma\beta^2L\ell(W_{t-1})
\end{eqnarray*}
We are now dealing with $|W^i_{t+1} - W^i_t|^2$.
\begin{eqnarray*}
\lefteqn{\sum_{i=1}^n\left|W^i_{t+1} - W^i_t\right|^2} \\
& \leq & 3\sum_{i=1}^n\left|-\eta\sum_{k=1}^L F_{t,k+1}^i \left[F_{t,k+1}^i\right]^{\top}\left(W^i_{t} - \Phi_i\right)x_ix_i^{\top}\left[G_{t,k-1}^i\right]G_{t,k-1}^i + \nu\sum_{k=1}^L F_{t,k+1}^i\left(W_{t,k} - W_{t-1,k}\right)G_{t,k-1}^i\right|^2 \\
&   & + 3\eta^2\sum_{i=1}^n \left|\sum_{k=1}^L \sum_{j \neq i} F_{t,k+1}^i \left[F_{t,k+1}^j\right]^{\top}\left(W^j_{t+1} - \Phi_j\right)x_jx_j^{\top}\left[G_{t,k-1}^j\right]^{\top}G_{t,k-1}^i\right|^2 + 3\left|\Delta_{t,i}\right|^2 \\
& \leq & 6\eta^2\beta^4L^2\ell(W_t) + 3n\nu^2\beta^2|W_t - W_{t-1}|^2 \\
&      & -6\eta\nu\sum_{i=1}^n \sum_{k=1}^L\left\langle F_{t,k+1}^i\left[F_{t,k+1}^i\right]^{\top}\left(W_t^i - \Phi_i\right)\left[G_{t,k-1}^i\right]^{\top}G_{t,k-1}^i, \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i \right\rangle \\
&      & + 3n\eta^2L^2n^2\gamma^2\beta^4\ell(W_t) + \frac{6nL^4\beta^3\tau^2\nu^2}{\left(1 - L\sqrt{\beta}\tau\right)^2}|W_t - W_{t-1}|^2 + \frac{6nL^6\eta^2\beta^5\tau^2}{\left(1 - L\sqrt{\beta}\tau\right)^2}\ell(W_t) \\
& \leq & 7\eta^2\beta^4L^2\ell(W_t) + 4n\nu^2\beta^2|W_t - W_{t-1}|^2 \\
&      & -6\eta\nu\sum_{i=1}^n \sum_{k=1}^L\left\langle F_{t,k+1}^i\left[F_{t,k+1}^i\right]^{\top}\left(W_t^i - \Phi_i\right)\left[G_{t,k-1}^i\right]^{\top}G_{t,k-1}^i, \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i \right\rangle
\end{eqnarray*}
Since
\begin{eqnarray*}
\lefteqn{-\left\langle F_{t,k+1}^i\left[F_{t,k+1}^i\right]^{\top}\left(W_t^i - \Phi_i\right)\left[G_{t,k-1}^i\right]^{\top}G_{t,k-1}^i, \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i \right\rangle} \\
& \leq & -\alpha^2\left\langle W_t^i - \Phi_i,  \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i \right\rangle + \epsilon\alpha^2\sum_{k'=1}^L |W_t^i - \Phi_i|\left|F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i\right|\\
& \leq & -\alpha^2\left\langle W_t^i - \Phi_i,  \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i \right\rangle + \frac{\epsilon\alpha^2L}{2}|W_t^i - \Phi_i|^2 + \frac{\epsilon\alpha^2\beta^2L}{2}\left|W_{t} - W_{t-1}\right|^2 \\
& \leq & -\alpha^2\left\langle W_t^i - \Phi_i,  W^i_t - W^i_{t-1} \right\rangle + \frac{\epsilon\alpha^2L}{2}|W_t^i - \Phi_i|^2 + \frac{\epsilon\alpha^2\beta^2L}{2}\left|W_{t} - W_{t-1}\right|^2 \\
&      & + \alpha^2|W_t^i - \Phi_i|\left|W^i_t - W^i_{t-1} - \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i\right| \\
& \leq & \alpha^2\left(\frac{1}{2}|W_{t-1}^i - \Phi_i|^2 - \frac{1}{2}|W_{t}^i - \Phi_i|^2 - \frac{1}{2}|W_t^i - W_{t-1}^i|^2\right)+ \frac{\epsilon\alpha^2L}{2}|W_t^i - \Phi_i|^2 + \frac{\epsilon\alpha^2\beta^2L}{2}\left|W_{t} - W_{t-1}\right|^2 \\
&      & + \alpha^2|W_t^i - \Phi_i|\left|W^i_t - W^i_{t-1} - \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i\right|
\end{eqnarray*}
we have
\begin{eqnarray*}
\lefteqn{\sum_{i=1}^n \sum_{k=1}^L\left\langle F_{t,k+1}^i\left[F_{t,k+1}^i\right]^{\top}\left(W_t^i - \Phi_i\right)\left[G_{t,k-1}^i\right]^{\top}G_{t,k-1}^i, \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i \right\rangle} \\
& \leq & \frac{\alpha^2 L}{2}\ell(W_{t-1}) - \frac{\alpha^2L(1 - 2\epsilon L)}{2}\ell(W_t) + \frac{\epsilon n \alpha^2 \beta^2 L^2}{2}|W_t - W_{t-1}|^2 \\
&      & + \frac{n\alpha^2}{2\epsilon}\left|W^i_t - W^i_{t-1} - \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i\right|^2
\end{eqnarray*}
Since
\[
\left|W^i_t - W^i_{t-1} - \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i\right| \leq \frac{L\tau\beta|W_t - W_{t-1}|}{1 - L\tau\beta} \leq 2L\beta\tau|W_t - W_{t-1}|
\]
we have
\begin{eqnarray*}
\lefteqn{\sum_{i=1}^n \sum_{k=1}^L\left\langle F_{t,k+1}^i\left[F_{t,k+1}^i\right]^{\top}\left(W_t^i - \Phi_i\right)\left[G_{t,k-1}^i\right]^{\top}G_{t,k-1}^i, \sum_{k'=1}^L F_{t,k'+1}^i\left(W_{t,k'} - W_{t-1,k'}\right)G_{t,k'-1}^i \right\rangle} \\
& \leq & \frac{\alpha^2 L}{2}\ell(W_{t-1}) - \frac{\alpha^2L(1 - 2\epsilon L)}{2}\ell(W_t) + n\alpha^2\beta^2 L^2\left(\frac{\epsilon}{2}+\frac{\tau^2}{\epsilon}\right)|W_t - W_{t-1}|^2 \\
& \leq & \frac{\alpha^2 L}{2}\ell(W_{t-1}) - \frac{\alpha^2L(1 - 2\epsilon L)}{2}\ell(W_t) + n\alpha^2\beta^2\epsilon|W_t - W_{t-1}|^2
\end{eqnarray*}
and therefore
\begin{eqnarray*}
\lefteqn{\sum_{i=1}^n |W_{t+1}^i - W_t^i|^2} \\
& \leq & -\left(3\eta\nu\alpha^2 L(1 - 2\epsilon L) -7\eta^2\beta^4L^2\right)\ell(W_t) + 3\eta\nu\alpha^2L\ell(W_{t-1}) + \left(4n\nu^2\beta^2 + n\eta\nu\alpha^2\beta^2\epsilon\right)|W_t - W_{t-1}|^2 \\
& \leq & - 3\eta\nu\alpha^2 L (1 - 3\epsilon L)\ell(W_t) + 3\eta\nu\alpha^2L\ell(W_{t-1}) + 8n\nu^2\beta^2|W_t - W_{t-1}|^2
\end{eqnarray*}
Finally, we have
\begin{eqnarray*}
\lefteqn{\ell(W_{t+1}) - \ell(W_t) \leq  \left(4n\nu^2\beta^2 + \frac{n\nu}{\eta}\right)|W_t - W_{t-1}|^2 } \\
&  & - \left(\frac{3}{2}\eta\nu\alpha^2 L (1 - 3\epsilon L)  - \frac{\eta\alpha^2 L}{2} + 3n\eta\gamma\beta^2L\right) \ell(W_t) + \left(\frac{3}{2}\eta\nu\alpha^2L+n\eta\gamma\beta^2L\right)\ell(W_{t-1})
\end{eqnarray*}
Using the inequality
\[
|W_{t+1} - W_t|^2 \leq \left(\nu^2 + 4\eta\nu\beta^2\tau \right)|W_t - W_{t-1}|^2 - 2\eta\left(\nu - \eta \beta^2 L\right)\ell(W_t) + 4\eta\nu\ell(W_{t-1})
\]
we have
\begin{eqnarray*}
\lefteqn{\ell(W_{t+1}) + \underbrace{\theta\left(4n\nu^2\beta^2 + \frac{n\nu}{\eta}\right)}_{:=b}|W_{t+1} - W_{t}|^2 } \\
& \leq & \underbrace{\left(4n\nu^2\beta^2 + \frac{n\nu}{\eta}\right)\left(1 + \theta\left(\nu^2 + 4\eta\nu\beta^2\tau \right)\right)}_{:=c}|W_t - W_{t-1}|^2 \\
&  & + \underbrace{\left\{1 - \left(\frac{3}{2}\eta\nu\alpha^2 L (1 - 3\epsilon L)  - \frac{\eta\alpha^2 L}{2} + 3n\eta\gamma\beta^2L - 2\theta\eta\left(4n\nu^2\beta^2 + \frac{n\nu}{\eta}\right)\left(\nu - \eta \beta^2 L\right)\right)\right\}}_{:=a_1} \ell(W_t) \\
&  & + \underbrace{\left(\frac{3}{2}\eta\nu\alpha^2L+n\eta\gamma\beta^2L+4\theta\eta\nu\left(4n\nu^2\beta^2 + \frac{n\nu}{\eta}\right)\right)}_{:=a_2}\ell(W_{t-1})
\end{eqnarray*}
Hence, according to Lemma 1 from ``Global convergence of the Heavy-ball method for convex optimization'', we have
\[
    \ell(W_{t+1}) \leq (1 - q)^t(q - a_1 + 1)\ell(W_1)
\]
where
\[
q = \max\left(\frac{c}{b}, \frac{a_1 + \sqrt{a_1^2 + 4a_2}}{2}\right)
\]
Since
\[
\frac{a_1 + \sqrt{a_1^2 + 4a_2}}{2} \leq \frac{1}{2}\left(a_1 + 2 - a_1 -\sqrt{1 - a_1 - a_2} \right) \leq 1 - \frac{1}{2}\sqrt{1 - a_1 - a_2}
\]
and
\[
1 - a_1 - a_2 = \frac{\eta\nu\alpha^2L}{2}\left(1 - 9\nu\epsilon L\right) - 4n\eta\gamma\beta^2L - 2\theta\eta\left(4n\nu^2\beta^2 + \frac{n\nu}{\eta}\right)\left(\nu + \eta\beta^2L\right)
\]
by choosing small enough $\nu = O(1/n)$, we have
\[
    1 - a_1 - a_2 \leq O\left(\eta\alpha^2 L\right)
\]
By choosing $\theta = 1 - \sqrt{1 - a_1 - a_2}/2$, we have $q \leq 1 -  \Omega(\sqrt{\eta\alpha^2 L})$.


==> old_snapshots/NTK-20201209.tex <==
\section{Neural Tangent Kernel Equivalence} \label{sec:NTK}
Lemma~\ref{lemma:tao_bound} bounds the maximal variation of the network's layers with probability of at least $1 - \exp(-\Omega(\sqrt{m}))$ as follows, 
\begin{eqnarray} \label{def:xi_ntk}
\tau = \max\limits_{1 \leq t \leq T}\max\limits_{k\in [L]} \nm{W_{t,k}-W_{1,k}}_2 \leq O\left(\frac{\beta \sqrt{\ell(W_1)}   }{\alpha^2 L}\right)=O\left(\frac{d_y(nd_x)^{1/2}m^{-1/2}}{L}\right)
 \vcentcolon= \frac{\xi}{L}
\end{eqnarray}
For some small number $\xi(m;n,d_x,d_y)$. Let $\bar{W} = (\bar{W}_{1}, \ldots, \bar{W}_{L})$ be any solution which satisfies,
\begin{eqnarray*}
\nm{\bar{W}_{k}-W_{1,k}}_2\leq\xi L^{-1}~,~\forall {k\in [L]}
\end{eqnarray*}
Denote the difference $W'=\bar{W}-W_1$, and notice that $\nm{W'}_2\leq \xi$.\\
Define the Neural Tangent Kernel (NTK) and the NTK objective~\cite{jacot2018neural,allen2019convergence} of the initialized network for the $p$-th output, $p\in[d_y]$,  respectively,
\begin{eqnarray}
K_p^{\textrm{NTK}}(x_i, x_j) \vcentcolon= \langle \nabla y_p(x_i,W_1),\nabla y_p(x_j,W_1)\rangle \quad,\quad 
y_p^{\textrm{NTK}}(x_i,W')=\langle \nabla y_p(x_i,W_1),W' \rangle
\end{eqnarray}
Jacot et al.~\cite{jacot2018neural}  proved that for an \textit{infinite} $m$, the dynamic NTK and NTK are in fact equivalent as $\varepsilon \rightarrow 0$. Allen-Zhu  et al.~\cite{allen2019convergence} showed a high-order polynomial bound on this equivalence. We further improve their results by stating a tighter bound on $m$ for our setting.
% We now improve the previously known equivalence between the dynamic NTK and the NTK at initialization described in~\cite{allen2019convergence}. 
%\asaf{TODO: change based on new result.}
% While previous $m$ is at least a high-order polynomial of $L$, we bound it with the data dimension $d$ alone, and the depth is actually \textit{reduces} the required width, i.w. $m=O\left( d^{1+\frac{1}{L}}\right)$. 
%\asaf{add conditions: 1. $\xi<<L^{3/2} so m>L^3$}
\begin{thm} \label{thm:NTK}
For every $x_i\in \R^d$, $1\leq p \leq d_y$, $W': \nm{W'}_2\leq \xi$ and $m=\Omega(n d_x d_y^2 L^3)$, with probability of at least $1-\exp(-\Omega(m))$ over the initialization of $\braces{B,C,\Psi,W_1}$ we have,
\begin{eqnarray}
\nm{\nabla y_p(x_i,W_1+W')-\nabla y_p^{\textrm{NTK}}(x_i,W')}_F \leq \mathcal{R} \nm{\nabla y_p^{\textrm{NTK}}(x_i,W')}_F
\end{eqnarray}
With the ratio,
\[\mathcal{R}= O\left(\frac{n^{1/2}d_x^{3/2}(L d_y)^2 }{m^{5/2}}\right)
\]
\end{thm}
\begin{cor} \label{thm:NTK_corollary}
For every $x_i,x_j\in \R^d$, $1\leq p \leq d_y$, $W': \nm{W'}_2\leq \xi$ and $m=\Omega(n d_x d_y^2 L^3)$ ,  with probability of at least $1-\exp(-\Omega(m))$,
\begin{eqnarray} \label{eqn:NTK_cor_main}
|\langle \nabla y_p(x_i,W_1+W'),\nabla y_p(x_j,W_1+W') \rangle- K_p^{\textrm{NTK}}(x_i, x_j) | \leq O\paren{\mathcal{R}} \sqrt{K_p^{\textrm{NTK}}(x_i, x_i) K_p^{\textrm{NTK}}(x_j, x_j)}
\end{eqnarray}
\end{cor}
Proofs can be found in Sections~(\ref{proof:thm_NTK}, \ref{proof:thm_NTK_cor}). Theorem~\ref{thm:NTK} guarantees that the difference between gradients is negligible with respect to their norms, thus the
NTK is a good approximation for the dynamic one. For simplicity we state the result per single output dimension $p$, while it holds for outputs of dimension $d_y$ as well.

For comparison, the corresponding ratio in~\cite{allen2019convergence} is significantly worse: $\frac{L^{3/2}}{\sqrt{\log m}}$. \\
More Specifically, equipped with the width required by theorem~\ref{thm:linear_rate_convergence}, the guaranteed ratio  by theorem~\ref{thm:NTK},
\[
\mathcal{R}=O\paren{n^{9/2}d_x^{7/2}d_y^{3}L^{1/2}}
\]
Finally, notice that the required width in theorem~\ref{thm:NTK}
is \textit{linear} in the number of training examples $n$, while previous works require high-order polynomial dependency. 
%Those properties are essentially related to the unique 
%\asaf{summarize and relate to generalization like allen.}
% -TODO: 
% -I differentiate by $k$. The full-grad is a vector of all the grads by $W_k$s, so I need to multiply by L (on both terms?). Also, move to full-grad in the theorem, and in the proof break it to k-s, and also if $d_y$>1, all generalize the same( allen used unit-vector). \\
%-Same for the $j$ in the theorem - can be moved to the proof. \\
% -Can compare the ratio with Allen - their maximal $\omega$ leads to a ration of: $\frac{L^{3/2}}{\sqrt{\log m}}$ \\
% -additional motivation for using gated-relu: gradients at initialization are more similar and can be used in NTK context. \\
% - Rearrange so no citation from the appendix of~(\ref{def:tau})'s value.\\
% - Note: Allen-Zhu's proof seems problematic - picking $\omega$ in their low range leads to NTK equivalency (a) of probability $1-\exp{O(1)}$. \\


==> old_snapshots/experiments-2020-12-09.tex <==
\section{Experiments} \label{sec:experiments}
In order to compare the proposed approach with the traditional ReLU one, we have implemented our Gated ReLU method in a fully connected network with different numbers of layers and channels per layer, and have compared the results with the exact same architecture using regular ReLU.
In this section, we address the following points:
\begin{itemize}
    \item How does the number of layers and channels impact the performance of our method ?
    \item How close to the theory are the practical hyper-parameters such as learning rate, number of steps, final MSE... ?
    \item Is our method limited to regression or can be extended to classification ?
    \item Can our method be an alternative to ReLU without any or just a few computational overhead?
\end{itemize}
We start with an experiment on a regression dataset, move to a synthetic dataset, and then show that this idea can also be applied in classification. In both cases, we try to vary the number of channels and layers to observe their impact on the convergence. 
\subsection{Implementation}
The implementation of Gated ReLU is quite simple, and can be described in Fig. \ref{fig:network_blocks}. It consists of two networks in parallel, that receive the same initialization procedure (with different random seeds), while the second (auxiliary) network controls the "gates" replacing the ReLU in the main network. The auxiliary network is not a strict copy of the main network since this would imply to multiply the computational complexity of the inference by 2. Instead, for every convolution layer in the main network that requires $(m\times m)$ operations, we associate to the auxiliary network a low rank approximation consisting of a succession of two FC layers with respective sizes $(m\times rm)$ and $(rm\times m)$ where $r$ is chosen to be $r=0.05$. In this setting, instead of using $m^2$ operations for every layer as it would be required if the auxiliary network would be similar to the main one, we have $2rm^2$ operations, that is only $10\%$ of the computations required by a regular FC network given the choice of $r$. Since the gates depend only on the output of the auxiliary network, and the theoretical and empirical ratio of such opened gates is 0.5, after we have ran an example inside the auxiliary network, we can predict in advance what channels have their output activated by the gates, and avoid to compute the ones whose associated gate is closed. In this setting, the main network requires just $50\%$ of the FLOPS required by a single ReLU network. In total, the computational complexity required by our method is $60\%$ of the one required by its ReLU counterpart, $10\%$ required by the auxiliary network, and $50\%$ by the main network given the fact that our matrix multiplications are sparse. 
\subsection{Regression}
\paragraph{SGEMM dataset}
Since our methods requires to have a high number of data samples, we choose the SGEMM GPU kernel performance Data Set, available online\footnote{\url{https://archive.ics.uci.edu/ml/datasets/SGEMM+GPU+kernel+performance}} with more than 241600 samples. We build a network using 10 FC layers with 4096 features. For both Gated ReLU and Regular ReLU experiments, we use the same initialization, and structure. 
We train our networks with different learning rates, both for the gated and regular ReLU, and present results in figures \ref{fig:train_loss_cst} and \ref{fig:train_loss_relu}. The chosen learning rate are the one that lead to a stable training, and the next that starts to show a problem of convergence. We can see that our method converges faster and is more stable allowing  higher learning rate. While our method can converge with a learning rate of $10^{-3}$, the maximum learning rate that would not lead to divergence for regular Relu is $10^{-4}$. When multiplying this latter by two, we can already see the training loss getting unstable.  In figure \ref{fig:train_loss_sgemm3}, we present the evolution of the loss when using same learning rate for both regular and gated ReLU's. We can observe that the gated ReLU network has a more stable training and converges faster to a lower MSE. In order to explain the reason for the fact that our method allows a higher learning rate, for every step, we compute the average absolute difference between the gradients of the current and previous step, and present this difference as function of a step in figure \ref{fig:train_loss_grad} both for our method and regular ReLU when using a stable learning rate for both methods of $10^{-4}$. The higher this difference, the less stable is the training, since it would imply that the gradients change a lot during the training. In figure \ref{fig:successive_relu_hamming}, we present the mean hamming distance between the activation pattern of the ReLU at two epochs. For this, we select a subset of input data, and record the pattern of the activated ReLU for the network at epoch $e$ and $e+1$, and compute the average hamming distance between them on all images, layers, and neurons in the network. Again, we can observe that as the training evolves, this activation pattern for ReLU network changes more and more, while it does not vary at all (by definition) for our Gated ReLU, that could explain the fact that the training is more stable, and that the gradients in our network vary less that the ones in the ReLU one. As predicted by Theorem \ref{thm:NTK}, {\color{blue} Yonathan: Asaf, please check this is the correct theorem}, we can observe that, unlike regular ReLU, this difference does not increase along the training and even get smaller, leading to a more stable training and allowing higher learning rates. 

Finally, we show the impact of the number of channels and layers in Figure \ref{fig:train_loss_sgemm2} {\color{blue} Yonathan: TODO, add latest graphs with more stable trainings. Currently running on hyper, will be ready by Tuesday morning}. As can be seen, it seems that our method performs better with deeper network than with shallower wider ones.
%We also use the highest possible learning rate that does not lead to divergence. For Gated ReLU; the learning rate is $7\cdot10^{-5}$ while for regular ReLU, the learning rate used is $2\cdot10^{-5}$.  In addition, we also compare the convergence of our network using the same learning rate as the regular ReLU one (even though the latter is not optimal for our metehod). We train the regression for 600 epochs, using SGD with Nesterov momentum set to $0.9$. Figure \ref{fig:train_loss_sgemm} shows the evolution of the MSE as a function of epochs. We can see that using gated Relu leads to faster convergence, but also to a lower MSE, not only using the maximum possible learning rate, but also using a lower learning rate that leads to more stable convergence. The fact that we do not reach zero error is because we do not train the network until full convergence, as the theory shows that this would require a significantly higher number of epochs. In addition, we show the impact of the number of channels and layers in Figure \ref{fig:train_loss_sgemm2}. As can be seen, it seems that our method performs better with deeper network than with shallower wider ones.


\begin{figure}[h]
    \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
            \includegraphics[width=\textwidth]{figures/train_err_sgemm_cst.pdf}
            \caption{Gated ReLU}
            \label{fig:train_loss_cst}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
         \centering
            \centering
    \includegraphics[width=\textwidth]{figures/train_err_sgemm_relu.pdf}
    \caption{Regular  ReLU}
    \label{fig:train_loss_relu}
    \end{subfigure}
    \caption{MSE as a function of epochs on SGEMM dataset}
\end{figure}



\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
            \includegraphics[width=\textwidth]{figures/train_err_sgemm_lr_1e2.pdf}
        \caption{lr=$10^{-2}$}
    \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
            \includegraphics[width=\textwidth]{figures/train_err_sgemm_lr_1e3.pdf}
        \caption{lr=$10^{-3}$}
    \end{subfigure}
         \begin{subfigure}[b]{0.32\textwidth}
         \centering
            \includegraphics[width=\textwidth]{figures/train_err_sgemm_lr_7e4.pdf}
        \caption{lr=$7\cdot 10^{-4}$}
    \end{subfigure}
    \caption{MSE as a function of epochs for regular and Gated ReLU on SGEMM dataset}
    \label{fig:train_loss_sgemm3}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics{figures/train_err_sgemm_different_sizes.pdf}
    \caption{MSE as a function of epochs, number of kernel and layers for Gated ReLU on SGEMM dataset}
    \label{fig:train_loss_sgemm2}
\end{figure}




\begin{figure}[h]
    \centering
    \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
    \includegraphics[width=\textwidth]{figures/train_err_sgemm_grad.pdf}
    \caption{Average temporal difference of gradient for regular and Gated ReLU on SGEMM dataset}
    \label{fig:train_loss_grad}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
         \centering
    \includegraphics[width=\textwidth]{figures/activation_relu.pdf}
    \caption{Average temporal hamming distance between successive binary ReLU's activation pattern}
    \label{fig:successive_relu_hamming}
    \end{subfigure}
    \caption{Evolution of gradients and activation patterns}
\end{figure}

\paragraph{Synthetic Dataset}
In this experiment, we generate a regression dataset using a explicit functional. Given a input vector $x\in\mathbb{R}^n$, the following mapping is applied: 
$$
f(x)=\sum_i x_{n-i}\left(\log{\left(|x_i|\right)\left(\cos(x_i)+x^3\sin(x)\right)}+\sqrt{|x|}\right)
$$
We choose a setting where the dimensionality of the input is 200, and generate 100.000 samples. We use the same architecture as in the previous paragraph, a 10 layer fully connected network with 4096 features in each layer. We try to compute the average MSE loss for several learning rates, both for our Gated ReLU and the regular ReLU. results are presented in Fig. \ref{fig:synthetic_loss}. Again we can see that not only our method has a more stable training and allows higher learning rates, but also, converges to zero MSE while regular ReLU does not reach it.


\begin{figure}[h]
    \centering
    \includegraphics{figures/train_err_synt.pdf}
    \caption{MSE as a function of epochs for regular and Gated ReLU on synthetic dataset}
    \label{fig:synthetic_loss}
\end{figure}
\subsection{Cifar 10}
We also implement our method on Cifar 10 dataset.
For all of our experiments, we train our networks on CIFAR10 datasets, from which every $(32\times 32 \times 3)$ input image is converted to a $3072$-dimensional normalized vector. We initialize the FC network as described in \ref{sec:preliminaries}. Every exeriment is conducted with the same hyper parameters. We train both networks with learning rate $10^{-4}$. Even though the Cifar dataset is a classification dataset, where the conventional loss is computed as a cross entropy between the softmax of the output logits and the true target, in our setting, we express the problem as a regression dataset and use a mean squared error between the output logits and the one-hot vector encoding the correct class.  Results are presented in the below table:

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
         Network architecture & train error with regular ReLU & train error with gated Relu \\ \hline
         6 layers, 10k channels & 0.48 & 0.02  \\ \hline
         7 layers, 10k channels & 0.27 & 0.01  \\ \hline
         4 layers, 15k channels & 0.75 & 0.03  \\ \hline
    \end{tabular}
    \caption{Training error for regular and Gated ReLU's on Cifar 10}
    \label{tab:experiment}
\end{table}

In figure \ref{fig:train_loss_cifar}, we show the evolution of the training loss as a function of epoch for Gated and Regular ReLU on CIFAR 10 using a FC network with 4 layers and 15k channels. We can see that the training loss of the Gated ReLU network converges to zero much faster that the one with Regular ReLU.
\begin{figure}[h]
    \centering
    \includegraphics{figures/train_err_cifar10.pdf}
    \caption{Training loss as a function of epochs for regular and custom ReLU}
    \label{fig:train_loss_cifar}
\end{figure}
\asaf{If we put a table (2) instead of graph it can contain: 1. test error (once, so we can focus on train-error in graphs. 2. FLOPS, so no one will miss the ~50 percent improvement :) \\
Synthetic - better cite something on the selected function. Also, not sure what is the point behind the current experiment (let's discuss).}
\subsection{Discussion}
Referring to table \ref{table:theo_comparison}, we can compute the theoretical number of neurons and learning rate required to reach zero accuracy. We can see that the learning rate we used in practice both for Cifar and SGEMM experiments is higher that the theoretical learning rate and that the number of neurons per layer is much smaller that the theoretical one. Yet, in CIFAR, it converged to a zero training error. We also notice that the pratical maximum learning rate is higher that the one of a regular ReLU network. {\color{Blue} Yonathan: This part is important, and we should focus here on all the conclusion that can be drawn from the experiment, as well as the comparison with the theory, even though we use hyperparameters that are different than the theoretical ones, yes, closer to them that to the one of previous work}
% \asaf{Suggested additions: \\
% \begin{enumerate}
%     %\item Accuracy of classification in CIFAR.
%     \item \sout{Experiment with output scaled *100, and discuss the flexibility allowed by our unique normalization}
%     \item \sout{Explain how gated-relu can be efficiently implemented. Discussing the time complexity is obligatory by the conference.}
%     \item \sout{In cifar - add the explanation of treating the classification as regression, it's good.}
%     \item \sout{For SGEMM, some discussion on the fact that it doesn't reach 0 error is needed. Maybe the order should be reversed: present cifar first (as regression with MSE + classification with CE), then "we wanted" to pick a natural regression with huge number of examples - we don't expect 0 error as $m$ not large enough, but still exhibit significantly improved results.."}
%     \item when stating the learning rate for the regular relu, can mention that we don't use their theory as in table 1 can be seen - it's impractical (like $O(10^{-100})$)
%     \item Niv: with an additional synthetic example can generate $n,d_x,d_y$ that distinct us from regular relus theory.
% \end{enumerate}}

==> old_snapshots/intro-2020-12-09.tex <==
\section{Introduction}
Deep neural networks have achieved a remarkable success in machine learning applications of different fields such as computer vision~\cite{voulodimos2018deep}, speech recognition~\cite{hinton2012deep} and natural language processing~\cite{devlin2018bert}. 
Much of this success in yet to be fully explained. \\
One of the existing gaps is referred to as the network \textit{trainability}, its ability to perfectly fit training data when initialized randomly and trained by first-order methods.
Modern deep networks are commonly equipped with rectified linear unit (ReLU) activations~\cite{xu2015empirical}, forming highly non-convex and non-smooth optimization problems. Such problems are known to be generally computationally infeasible~\cite{livni2014computational}, and NP-hard in some cases~\cite{blum1989training}. Nevertheless, in practice, trainability is often achieved in various tasks. Such empirical findings were summarized by Zhang et al.~\cite{zhang2016understanding}:
"Deep neural networks easily fit (random) labels".

Previous theoretical works focused on networks \textit{expressivity}~\cite{bengio2011expressive,cohen2016expressive}, the existence of a solution that perfectly fits training data, therefore necessary for trainability. As it has been shown that even shallow networks are universal approximators~\cite{hornik1989multilayer}, a better understanding of the power of depth was desired~\cite{eldan2016power,liang2016deep,telgarsky2015representation}.
%[h [13, 17, 30, 33, 37, 38, 44, 45, 49, 50-memorizers,,nadav].
One conclusion is that increased depth allows exponentially more efficient representations, thus per parameter, deep networks can approximate a richer class of functions than shallow ones~\cite{cohen2016expressive,liang2016deep}. \\
However, a recent work~\cite{yun2019small} provided tighter expressivity bounds on ReLU networks, showing that datasets of $n$ training examples can be perfectly expressed by a $3$-layer ReLU network with $\Omega{\paren{\sqrt{n}}}$ parameters. This is inconsistent with
the sizes of practical neural networks that typically exceed the size of the training data. This regime is often referred to as \textit{overparameterization}.
It appears that expressivity can provide only a limited explanation for the overparameterization of modern neural networks, which keep growing deeper and wider in search of state-of-the-art results~\cite{zagoruyko2016wide,huang2019gpipe,ridnik2020tresnet}. 

Important insights regarding trainability emerged from analysis of simplified variants of neural networks.
Deep linear networks are of special interest as increased depth does not affect their expressiveness, only changes their optimization landscape. Therefore the effects of increased width and depth on the training process can be isolated and carefully studied in this setting. Arora et al.~\cite{arora2018convergence} proved that trainability is attained at a linear rate under proper initialization as long as the network is wide enough. %minimal width
Cohen et al.~\cite{arora2018optimization} showed that the process of training with gradient-descent can be accelerated by increasing the depth of the network. Their empirical evaluations supported the existence of a similar outcome in deep nonlinear networks as well.

Another line of active research with further insights is overparameterized shallow nonlinear networks, typically with a single hidden layer.
Du et al.~\cite{du2018power} proved that for a quadratic activation function all local minima are global minima.
Safran et al.~\cite{safran2018spurious}
showed that ReLU networks suffer from spurious local minima, which can be drastically reduced by overparameterization.
Oymak et al.~\cite{oymak2020towards} achieved trainability where the proportion between the number of hidden units and training examples $n$ depends on the activation: for smooth ones it is $\Omega\paren{n^2}$ while for ReLU it is significantly larger, $\Omega\paren{n^4}$. Additional works examined the unique dynamics of ReLU activation along the training and their relation to gradient-descent optimization~\cite{li2018learning,arora2019fine}.

The analysis of deep ReLU networks is more challenging, as additional problems emerge with increased depth. Exploding and vanishing gradient~\cite{hanin2018neural} and bias shifts~\cite{clevert2015fast} are shared with additional activations, while the dying ReLUs problem, causing them to remain inactive permanently, is unique~\cite{lu2019dying}.
While in practice those problems are solved by introduction of additional tensor transformations~\cite{ioffe2015batch, he2016identity}, their theoretical understanding remains limited. % missing 'surprisingly'!
% Correspondingly, existing bounds on the required overparameterization for trainability of deep fully-connected ReLU networks are far more loose than those achieved on shallow ones. 

Correspondingly, existing trainability guarantees for deep feed-forward ReLU networks are considerably weaker compared with shallow networks.
%than those achieved on shallow ones. 
Du et al.~\cite{du2019gradient} requires a minimal network width which scales exponentially with its depth $L$ and polynomially  with the number of examples $n$. More recent works~\cite{zou2018stochastic,allen2019convergence} improved the dependencies to be high-order polynomials, $\Omega\paren{n^{26}L^{38}}$ and $\Omega\paren{n^{24}L^{12}}$ correspondingly. 
% The best
% known result was established in~\cite{zou2019improved}, with required network width of $\Omega\paren{n^{8}L^{12}}$, 
The best known result by Zou et al.~\cite{zou2019improved} requires a network width of $\Omega\paren{n^{8}L^{12}}$, 
which is still prohibitively large compared to practice. 
For instance, training the common ImageNet dataset~\cite{krizhevsky2017imagenet} with ResNet-$1001$ architecture~\cite{he2016identity} requires a network of $\Omega\paren{10^{172}}$ parameters, while the largest one ever trained contains only $O\paren{10^{11}}$~\cite{brown2020language}.
% More specifically, for a standard training of the common ImageNet dataset~\cite{krizhevsky2017imagenet} with ResNet-$1001$ architecture~\cite{he2016identity}, the required number of parameters is $\Omega\paren{10^{172}}$ while the largest network ever trained is contain only $\Omega\paren{10^9}$ parameters. 

In this paper we take a step towards closing the gap between theory and practice. We develop a simplified analysis for the trainability of overparameterized deep neural networks, which significantly improves previous guarantees on their size.
The network width required by our analysis for trainability scales \textit{quadratically} with $n$, enabling an empirical verification for the first time, and bridging previous empirical results related to overparameterization. %TODO: improve.
In addition, the required width by our theory is \textit{linear} with $L$, paving the way for better understanding of the behaviour of deep neural networks of practical depths. 
Finally, the number of training iterations for reaching global minima by our theory is \textit{linear} in $n$, significantly smaller than previous results. %$O\paren{n L^{1/2}}$ 
A full comparison with previous methods can be found in table~\ref{table:theo_comparison}.

A key novelty of our approach is the fixed ReLU activation pattern of the network. The activations patterns, i.e. which entries output zero~\cite{hanin2019deep}, are set during initialization - permanently. 
They are set based on a random fixed transformation of the input, independent of the network initialization, therefore, immune to dying ReLUs and bias shifts while enjoying the advantages of ReLU activation.
% While enjoying the advantages of ReLU activation, the proposed network does not suffer from dying ReLUs or bias shifts.
% Previous works showed that the number of activation patterns is surprisingly small~\cite{hanin2019deep} and reduced by overparameterization~\cite{li2018learning}. We fix

The remainder of this paper is organized as follows. In section~\ref{sec:preliminaries} we state the problem setup notational conventions. Our main theoretical result is covered in section~\ref{sec:main_theory}, and followed by an improved analysis for Neural Tangent Kernel in section~\ref{sec:NTK}. In section~\ref{sec:experiments} we empirically demonstrate the properties and  effectiveness of the proposed theory. Section~\ref{sec:related} contains additional related work. Finally, section~\ref{sec:conclusion} concludes our work.

\begin{figure}[h]    
          \centering
        \includegraphics[width=\linewidth]{figures/gated_relu.pdf}
        % \caption{A naive implementation of the suggested network. Blue layers are trained while red ones set the activations and are kept fixed during the training.}
        % \label{fig:network_blocks}
        \caption{Sketch of the proposed network. Blue layers are trained while red layers set the activations and remain unchanged during training. Efficient implementation reduces both training and inference times by almost $50\%$.}
        \label{fig:network_blocks}
\end{figure}
% are --- the ones of shallow networks.
% trainability becomes more challenging.
%require unrealistic over-parameterization conditions
%on the width of neural networks, especially for deep networks
%small change to relu - much stronger convergence.
% When deeper models are considered, additional problems emerge in ReLU networks trained with first-order methods. The exploding and vanishing gradient problem is increased with depth~\cite{hanin2018neural}. 
% Correspondingly, the -- trainability becomes more challenging.
% \cite{oymak2020towards} proved that overparameterized networks with a single hidden layer are trainable for structured data as long as the number of hidden neurons $m$ is proportional to $O(n^4)$

% --- practitioners use deep/(when pram>data).. ..."What is the amount and kind of overparameterization that enables trainability?"

% When general deep networks are considered, results are (weaker../prohibitively large))




% typically 


% ..provided further insights(shallow, $1$-hidden).
 


%summarize: cannot generalize to DNNs with relu.
% like shallow relu networks~\cite{du2018power,safran2018spurious} and deep linear networks~\cite{arora2018convergence}.

%the fact that practical neural networks are \textit{overparameterized}, with a number of parameters exceeds the size of the training data.


% Difficulties in optimizing deeper networks have also
% been long clear – the signal held by a gradient gets buried
% as it propagates through many layers. This is known as
% the “vanishing/exploding gradient problem”. Modern techniques such as batch normalization (Ioffe & Szegedy, 2015)
% and residual connections (He et al., 2015) have somewhat
% alleviated these difficulties in practice
%Another work~\cite{hanin2019deep} demonstrated that the number of activation regions actually learned in practice is 
% \newline 
% Paragraphs:
% \begin{itemize}
%     \item deep learning is great. Has remarkable ability to fit training data although objective is highly non-convex.
%     \item relu activation is widely used.Shown to lead to vanishing gradients, dead neurons~\cite{lu2019dying} and bias shifts..all affect when $L$ is large (depends on our experiments)
%     \item previous works.. towards bridging this gap between application and theory. Cite the work with bad results on overparameterized, and say that with tighter bounds we can harness theoretical improvements to empirical ones + understand why narrower nets work better. 
%     \item Allen claimed that he proved that Residuals are not a must - but we show it for practical uses (read Du's paragraph on that and refer as well). Our width and number of iterations does not depend on $L$.
%     \item empathize that first to overparameterize with weak dependency on the depth, while \cite{du2019gradient}-exponential,and \cite{allen2019convergence} polynomial (done only in 2-3 layers and deep linear networks).
%     \item our network is more flexible to labels range. While previous work assumed $y=O(1)$, we can. assume $y=O(m)$. Specifically the bounds in \cite{allen2019convergence} grow polynomially in $\Omega$ if $\|y\|\leq \Omega$ (footnote 6).
%     \item can mention that while in previous works precise normalization was crucial, we enjoy a freedom due to separability between gates and training - we get the same order of bound for different normalization of the final layer.
% \end{itemize}


==> old_snapshots/intro-20203011.tex <==
\section{Introduction}
Deep neural networks have achieved a remarkable success in machine learning applications of different fields such as computer vision~\cite{voulodimos2018deep}, speech recognition~\cite{hinton2012deep} and natural language processing~\cite{devlin2018bert}. 
Much of this success in yet to be fully explained. \\
One of the existing gaps is referred to as the network \textit{trainability}, its ability to perfectly fit training data when initialized randomly and trained by first-order methods.
Modern deep networks are commonly equipped with rectified linear unit (ReLU) activations~\cite{xu2015empirical}, forming highly non-convex and non-smooth optimization problems. Such problems are known to be generally computationally infeasible~\cite{livni2014computational}, and NP-hard in some cases~\cite{blum1989training}. Nevertheless, in practice, trainability is often achieved in various tasks. Such empirical findings were summarized by Zhang et al.~\cite{zhang2016understanding}:
"Deep neural networks easily fit (random) labels".

Previous theoretical works focused on networks \textit{expressivity}~\cite{bengio2011expressive,cohen2016expressive}, the existence of a solution that perfectly fits training data, therefore necessary for trainability. As it has been shown that even shallow networks are universal approximators~\cite{hornik1989multilayer}, a better understanding the power of depth was desired~\cite{eldan2016power,liang2016deep,telgarsky2015representation}.
%[h [13, 17, 30, 33, 37, 38, 44, 45, 49, 50-memorizers,,nadav].
One conclusion is that increased depth allows exponentially more efficient representations, thus per parameter, deep networks can approximate a richer class of functions than shallow ones~\cite{cohen2016expressive,liang2016deep}. \\
However, a recent work~\cite{yun2019small} provided tighter expressivity bounds on ReLU networks, showing that datasets of $n$ training examples can be perfectly expressed by a $3$-layer ReLU network with $\Omega{\paren{\sqrt{n}}}$ parameters. This is inconsistent with
the sizes of practical neural networks that typically exceed the size of the training data. This regime is often referred to as \textit{overparameterization}.
It appears that expressivity can provide only a limited explanation for the overparameterization of modern neural networks, which keep growing deeper and wider in search of state-of-the-art results~\cite{zagoruyko2016wide,huang2019gpipe,ridnik2020tresnet}. 

Important insights regarding trainability emerged from analysis of simplified variants of neural networks.
Deep linear networks are of special interest as increased depth does not affect their expressiveness, only changes their optimization landscape. Therefore the effects of increased width and depth on the training process can be isolated and carefully studied in this setting. Arora et al.~\cite{arora2018convergence} proved that trainability is attained at a linear rate under proper initialization as long as the network is wide enough. %minimal width
Cohen et al.~\cite{arora2018optimization} showed that the process of training with gradient-descent can be accelerated by increasing the depth of the network. Their empirical evaluations supported the existence of a similar outcome in deep nonlinear networks as well.

Another line of active research with further insights is overparameterized shallow nonlinear networks, typically with a single hidden layer.
Du et al.~\cite{du2018power} proved that for a quadratic activation function all local minima are global minima.
Safran et al.~\cite{safran2018spurious}
showed that ReLU networks suffer from spurious local minima, which can be drastically reduced by overparameterization.
Oymak et al.~\cite{oymak2020towards} achieved trainability where the proportion between the number of hidden units and training examples $n$ depends on the activation: for smooth ones it is $\Omega\paren{n^2}$ while for ReLU it is significantly larger, $\Omega\paren{n^4}$. Additional works examined the unique dynamics of ReLU activation along the training and their relation to gradient-descent optimization~\cite{li2018learning,arora2019fine}.

The analysis of deep ReLU networks is more challenging, as additional problems emerge with increased depth. Exploding and vanishing gradient~\cite{hanin2018neural} and bias shifts~\cite{clevert2015fast} are shared with additional activations, while the dying ReLUs problem, causing them to remain inactive permanently, is unique~\cite{lu2019dying}.
While in practice those problems are solved by introduction of additional tensor transformations~\cite{ioffe2015batch, he2016identity}, their theoretical understanding remains limited. % missing 'surprisingly'!
% Correspondingly, existing bounds on the required overparameterization for trainability of deep fully-connected ReLU networks are far more loose than those achieved on shallow ones. 

Correspondingly, existing trainability guarantees for deep feed-forward ReLU networks are considerably weaker compared with shallow networks.
%than those achieved on shallow ones. 
Du et al.~\cite{du2019gradient} requires a minimal network width which scales exponentially with its depth $L$ and polynomially  with the number of examples $n$. More recent works~\cite{zou2018stochastic} improved the dependencies to be high-order polynomials, $\Omega\paren{n^{26}L^{38}}$ and $\Omega\paren{n^{24}L^{12}}$ correspondingly. 
% The best
% known result was established in~\cite{zou2019improved}, with required network width of $\Omega\paren{n^{8}L^{12}}$, 
The best known result by Zou et al.~\cite{zou2019improved} requires a network width of $\Omega\paren{n^{8}L^{12}}$, 
which is still prohibitively large compared to practice. 
For instance, training the common ImageNet dataset~\cite{krizhevsky2017imagenet} with ResNet-$1001$ architecture~\cite{he2016identity} requires a network of $\Omega\paren{10^{172}}$ parameters, while the largest one ever trained contains only $O\paren{10^{11}}$~\cite{brown2020language}.
% More specifically, for a standard training of the common ImageNet dataset~\cite{krizhevsky2017imagenet} with ResNet-$1001$ architecture~\cite{he2016identity}, the required number of parameters is $\Omega\paren{10^{172}}$ while the largest network ever trained is contain only $\Omega\paren{10^9}$ parameters. 

In this paper we take a step towards closing the gap between the theory and practice. We develop a simplified analysis for the trainability of overparameterized deep neural networks, which significantly improves previous guarantees on their size.
The network width required by our analysis for trainability scales \textit{quadratically} with $n$, enabling an empirical verification for the first time, and bridging previous empirical results related to overparameterization. %TODO: improve.
In addition, the required width by our theory is \textit{linear} with $L$, paving the way for better understanding of the behaviour of deep neural networks of practical depths. 
Finally, the number of training iterations for reaching global minima by our theory is significantly smaller than previous results. %$O\paren{n L^{1/2}}$ 
For a full comparison with previous methods see table~\ref{table:theo_comparison}. 

A key novelty of our approach is the fixed ReLU activation pattern of the network. Activations patterns, i.e. whether each output equals the input or zero, are set during activation, permanently. 
They are set based on random a transformation of the network's input, independently of the network layers' initialization. 
% Previous works showed that the number of activation patterns is surprisingly small~\cite{hanin2019deep} and reduced by overparameterization~\cite{li2018learning}. We fix

The remainder of this paper is organized as follows. In section~\ref{sec:preliminaries} we state the problem setup and the notations used. Our main theoretical result is covered in section~\ref{sec:main_theory}, and followed by an extension for neural tangent Kernel in section~\ref{sec:NTK}. In section~\ref{sec:experiments} we empirically demonstrate the properties and  effectiveness of the proposed theory. Section~\ref{sec:related} contains additional related work. Finally, section~\ref{sec:conclusion} concludes our work.

% are --- the ones of shallow networks.
% trainability becomes more challenging.
%require unrealistic over-parameterization conditions
%on the width of neural networks, especially for deep networks
%small change to relu - much stronger convergence.
% When deeper models are considered, additional problems emerge in ReLU networks trained with first-order methods. The exploding and vanishing gradient problem is increased with depth~\cite{hanin2018neural}. 
% Correspondingly, the -- trainability becomes more challenging.






% \cite{oymak2020towards} proved that overparameterized networks with a single hidden layer are trainable for structured data as long as the number of hidden neurons $m$ is proportional to $O(n^4)$

% --- practitioners use deep/(when pram>data).. ..."What is the amount and kind of overparameterization that enables trainability?"

% When general deep networks are considered, results are (weaker../prohibitively large))




% typically 


% ..provided further insights(shallow, $1$-hidden).
 


%summarize: cannot generalize to DNNs with relu.
% like shallow relu networks~\cite{du2018power,safran2018spurious} and deep linear networks~\cite{arora2018convergence}.

%the fact that practical neural networks are \textit{overparameterized}, with a number of parameters exceeds the size of the training data.


% Difficulties in optimizing deeper networks have also
% been long clear – the signal held by a gradient gets buried
% as it propagates through many layers. This is known as
% the “vanishing/exploding gradient problem”. Modern techniques such as batch normalization (Ioffe & Szegedy, 2015)
% and residual connections (He et al., 2015) have somewhat
% alleviated these difficulties in practice


%Another work~\cite{hanin2019deep} demonstrated that the number of activation regions actually learned in practice is 



















\newpage

























% \newline 
% Paragraphs:
% \begin{itemize}
%     \item deep learning is great. Has remarkable ability to fit training data although objective is highly non-convex.
%     \item relu activation is widely used.Shown to lead to vanishing gradients, dead neurons~\cite{lu2019dying} and bias shifts..all affect when $L$ is large (depends on our experiments)
%     \item previous works.. towards bridging this gap between application and theory. Cite the work with bad results on overparameterized, and say that with tighter bounds we can harness theoretical improvements to empirical ones + understand why narrower nets work better. 
%     \item Allen claimed that he proved that Residuals are not a must - but we show it for practical uses (read Du's paragraph on that and refer as well). Our width and number of iterations does not depend on $L$.
%     \item empathize that first to overparameterize with weak dependency on the depth, while \cite{du2019gradient}-exponential,and \cite{allen2019convergence} polynomial (done only in 2-3 layers and deep linear networks).
%     \item our network is more flexible to labels range. While previous work assumed $y=O(1)$, we can. assume $y=O(m)$. Specifically the bounds in \cite{allen2019convergence} grow polynomially in $\Omega$ if $\|y\|\leq \Omega$ (footnote 6).
%     \item can mention that while in previous works precise normalization was crucial, we enjoy a freedom due to separability between gates and training - we get the same order of bound for different normalization of the final layer.
% \end{itemize}


% In this work, we develop a simplified analysis for overparameterized deep neural network. 
% \{1: previous works are based on the commonly used relu activation... which shown to lead to vanishing gradients, dead neurons~\cite{lu2019dying} and bias shifts..\} {2: previous bounds are prohibitively large to allow empirical verification, not to mention providing a theoretical justification to the ability of gradient-based optimization to solve highly non-convex problems as in deep learning.}\\
% There are $2$ key difference between this work and previous ones:

% \begin{enumerate}
%     \item The activations in this work are set once during the initialization, and \emph{remain unchanged} along the training. 
%     \item The activations are set based on randomly initialized pseudo-layers, which are independent of the initialization of the actual layers.  
    

% \end{enumerate}
% % One of the key difference between this work and previous ones is that the activations in this work are set once during the initialization, and \emph{remain unchanged} through the training. 
% % Additionally, activations are set by random projections which are independent of the layers initialization. 
% Based on those $2$ novelties, our analysis provides a significantly tighter lower-bound on the network's width than previous works. 

% \{In fact, it offers a theoretical justification.., practical use..\} 
% \{More specifically, previous bound $m>O\paren{(nL)^{30}}$~\cite{allen2019convergence} while ours $m>O\paren{n^{\frac{4}{3}}}$\}   


==> old_snapshots/main-20200905.tex <==
 \subsection{Discussion}
  Add a table with:
  \begin{itemize}
    \item Minimal width dependency on n,L. 
     \item error probability 
     \item assumptions on data
     \item number of iterations (linear convergence rate): Allen- $O\left(\frac{n^6L^2}{\delta^2\log(\frac{1}{\varepsilon})})\right)$
     \item NTK related size.
     \item learning rate(?)
     \item possibly we are not bounded to $y=O(1)$ while Allen does?
 \end{itemize}
% 
% Du: $$poly(n, 2^{O(L)}
% , 1/\lambda_{min}) $$
\begin{table}[t]
  \centering
  \setlength{\tabcolsep}{2pt}
  \resizebox{\linewidth}{!}{
  \scalebox{0.03}{
   \begin{tabular*}{0.5\textwidth}{l @{\extracolsep{\fill}} c c c c c}
    \toprule
    Work & Iterations & Neurons & Probability & learn-rate \\
    \midrule
    Du~\cite{du2019gradient} & 1 & 2 & 3 & 4  \\
    Allen-Zhu~\cite{allen2019convergence} & $\Theta\left(\frac{n^6L^2}{\delta^2\log(\frac{1}{\varepsilon})})\right)$ & $\Omega \left(\frac{n^{24}L^{12}d\log^5m}{\delta^8} \right)$              & $O\left( \exp\paren{-\log^2 m}\right)$ & $\Theta\left(\frac{\delta^9}{n^{28}\log^5m L^{14}}  \right)$   \\
    Other1 & 1 & 2 & 3 & 4  \\ \midrule
    Ours & $O\left(\frac{n^4}{d^2} \log\frac{1}{\varepsilon}\right)$ & $\Omega\left(\max\braces{n^2,n^{\frac{2}{3}}d^{\frac{4}{3}}}\right)$ & $O\left(\exp(-\Omega(\sqrt{m})\right)$ & $\Theta\left(\frac{d^4}{n^8L}\right)$  \\
    \bottomrule
  \end{tabular*}
  } }
%  \caption{caption}
%mention in caption that Du's activation are only smooth.
  \label{table:EfficientNet}
\end{table}


==> old_snapshots/preliminaries-2020-12-09.tex <==
\section{Preliminaries} \label{sec:preliminaries}
In this section we introduce the problem and the setup used to prove the main theory. %notations, data, network, W, loss.
\subsection{Notations} 
We begin by establishing notational conventions that will be used throughout the paper. 
We denote the Euclidean norm of vector $v$ by $\nm{v}$ or $\nm{v}_2$, and the Kronecker product and Frobenius inner-product for matrices $M,N$ by $M\otimes N$, $\langle M,N \rangle$ respectively. We denote by $\lambda_{\min}(M)$, $\lambda_{\max}(M)$ matrix minimal and maximal eigenvalues.  
We use the shorthand $[k]$ to denote the set $\{1,\dots,k\}$ and its positive part  by $[k]_+=\max(0,k)$ .Matrix column-wise vectorization is denoted by $\mbox{vec}\left(\right)$. Finally, we denote the normal and chi-square distributions by $\N(\mu, \Sigma),\chi^2_{d}$. 
% Let $\braces{(x_i, y_i = \Phi_i x_i)}_{i\in[n]}$, be training examples, with $\Phi_i \in \R^{d_y\times d_x}$, $x_i\in \R^{d_x}, y_i \in \R^{d_y}$. Note that a different linear mapping $\Phi_i$ is used for each training example as our goal is to fit a nonlinear objective $y_i$. We assume without loss of generality that input data is normalized, $\nm{x_i}=1$, and
% similar to previous works~\cite{allen2019convergence,li2018learning} we make the following assumptions on the data.
% \begin{assumption}[non-degenerate input]
% Every two distinct examples $x_i,x_j$ satisfy  $\|x_i^\top x_j\|\leq \delta$. %$\delta \ll 1$
% \end{assumption} 
% % \begin{assumption}[common regression labels] \label{assum:labels}
% % Training labels dimension and values are bounded: $d_y\leq M$, $\max_i|y_i|\leq M$,  for some constant $M$.
% % \end{assumption} 
% % \begin{assumption}[common regression labels] \label{assum:labels}
% % Labels are bounded: $\max_i|y_i|\leq M$,  for a constant $M$.
% % \end{assumption} 
% \begin{assumption}[common regression labels] \label{assum:labels}
% Labels are bounded: $\max_i|y_i|\leq O(\sqrt{m})$.
% \end{assumption}
% %\asaf{consider removing the $d_y<M$}
% Both assumptions hold for typical datasets, and are stated in order to simplify the derivation. In addition, assumption~\ref{assum:labels} is more relaxed than corresponding assumptions in previous works, typically $\max_i|y_i|\leq O(1)$, making it handle better large outputs as we shall demonstrate in the experiments section. 
%%%
%%%
\subsection{Problem Setup} %Fixed Activations
Let $\braces{(x_i, y_i = \Phi_i x_i)}_{i\in[n]}$, be training examples, with $\Phi_i \in \R^{d_y\times d_x}$, $x_i\in \R^{d_x}, y_i \in \R^{d_y}$. Note that a different linear mapping $\Phi_i$ is used for each training example as our goal is to fit a nonlinear objective $y_i$. We assume for convenience and without loss of generality that the input data is normalized, $\nm{x_i}=1$. The data is used for training a feed-forward neural network with $L$ hidden layers and $m$ neurons on each layer. It is defined and initialized as follows.
 All layers are initialized with independant Gaussian distributions,
\[
\brackets{W_k}_{i,j}\sim\N(0, 2/m)~~,
~~\brackets{\Psi_k}_{i,j}\sim\N(0, 2/m),
~~\brackets{C}_{i,j}\sim\N(0, 2/d_x),
~~\brackets{B}_{i,j}\sim\N(0, 2/d_y)
\]
The only trained layers are $W_{[L]}$, while $\paren{B,C,\Psi_{[L]}}$ remain unchanged during training. 
The activations $\{D^i_k, i \in [n], k\in [L]\}$ are computed based on the random weights of $\Psi_{[L]},B,C$ as follows,
\[
z^i_0 = [Cx_i]_+~~,~~z^i_k = [\Psi_k z_{k-1}^i]_+~~,~~  D_k^i = \mbox{diag}(z_k^i)~~~k=1,\ldots,L.
\]
Therefore do not change during training as well.
\autoref{fig:network_blocks} illustrate the described network. \\
We denote the $k$th layer at iteration $t$ by $W_{t,k}\in \R^{m\times m}$, and the concatenation of all trainable layers by $W_t = (W_{t,1}, \ldots, W_{t,L})$. Since the activations are fixed in time and change per example, the full network applied on example $i$ is the following matrix,
\[
    W_t^i \vcentcolon= BD_L^iW_{t,L}\ldots D_1^iW_{t,1}D_0^iC\in \R^{d_y\times d_x}
\]
% The activations in $D^i_k$ are induced by a separate set of random weights, denoted by $\Psi_k \in \R^{m\times m}, k\in [L]$, that play similar roles as $W_k, k \in [L]$. More specifically, each element in $\Psi_k, k\in [L]$ is sampled from Gaussian distribution $\N(0, 2/m)$, and $B,C$ elements are sampled from $\N(0, 2/(d_y)),\N(0, 2/d_x)$ respectively. 
% The activations in $\{D^i_k, i \in [n], k \in \{0,1,\ldots,L\}\}$ are computed based on the random weights in $\{\Psi_k, k \in [L]\}$, $B$ and $C$, i.e. $z^i_0 = [Cx_i]_+$, $z^i_k = [\Psi_k z_{k-1}^i]_+, k=1,\ldots, L$ and $D_k^i = \mbox{diag}(z_k^i)$. 
% It is important to note that weights in $B$, $\{\Psi_{k}, k \in [L]\}$ and $C$ remain unchanged during the optimization process, and so are activations in the diagonal matrices $\{D^i_k, i \in [n], k \in \{0,1,\ldots,L\}\}$. \autoref{fig:network_blocks} illustrate the described network. \\
% We assume that the network is \emph{overparameterized}:
% \begin{assumption}
% The network is overparameterized, that is $m=\Omega(nd)$. \label{assum:over} 
% \end{assumption} 
% Add: loss def- after explaining the freeze \ finish with it. \\
% define $F^i_{t,k}$ and state what's fixed.\\
% in the $D$s - explain the notation with the $[]_+$
% Using the above notation, given a solution $W_t = (C, W_{t,1}, \ldots, W_{t,L}, B)$, the overall $\ell_2$ loss function can be written as:
%See section~\ref{sec:init} for additional details. 
Following previous works~\cite{allen2019convergence,du2019gradient,oymak2020towards}, we focus on the task of regression with the square loss,
%optimize the square loss for a regression task,
\[
    \ell(W_t) = \frac{1}{2}\sum_{i=1}^n \nm{(W_t^i - \Phi_i)x_i}^2
\]
Our result can be extended to other tasks and loss functions such as classification with cross-entropy similarly to~\cite{allen2019convergence,zou2018stochastic} and omitted for brevity.
The loss is minimized by gradient-descent with a constant learning rate.
In addition, two important definitions for the analysis: \\
the intermediate transform for $1\leq k' \leq k \leq L$,
\begin{eqnarray}
Z^t_{k,k'} \vcentcolon= D_k^iW_{t,k}\ldots W_{t,k'+1}D_{k'}^i
\end{eqnarray}
and, the maximal variation from initialization of the network's trained layers,
\begin{eqnarray} \label{def:tau}
    \tau \vcentcolon= \max\limits_{1\leq t \leq T}\max\limits_{k \in [L]} \left\|W_{t,k} - W_{1,k}\right\|_2
\end{eqnarray}


% Define the intermediate transform for $1\leq k' \leq k \leq L$,
% \begin{eqnarray}
% Z^t_{k,k'} \vcentcolon= D_k^iW_{t,k}\ldots W_{t,k'+1}D_{k'}^i
% \end{eqnarray}
% Finally, define the maximal variation from initialization of the network's trained layers,
% \begin{eqnarray} \label{def:tau}
%     \tau \vcentcolon= \max\limits_{1\leq t \leq T}\max\limits_{k \in [L]} \left\|W_{t,k} - W_{1,k}\right\|_2
% \end{eqnarray}
%where $T$ is the number of iterations.
% \subsection{Network architecture and initialization} \label{sec:init}
% % The activations in $D^i_k$ are induced by a separate set of random weights, denoted by $\Psi_k \in \R^{m\times m}, k\in [L]$, that play similar roles as $W_k, k \in [L]$. More specifically, each element in $\Psi_k, k\in [L]$ is sampled from Gaussian distribution $\N(0, 2/m)$, and $B,C$ elements are sampled from $\N(0, 2/(d_y)),\N(0, 2/d_x)$ respectively. 
% % The activations in $\{D^i_k, i \in [n], k\in [L]$ are computed based on the random weights in $\{\Psi_k, k \in [L]\}$, $B$ and $C$, i.e. $z^i_0 = [Cx_i]_+$, $z^i_k = [\Psi_k z_{k-1}^i]_+, k=1,\ldots, L$ and $D_k^i = \mbox{diag}(z_k^i)$. 
% % It is important to note that weights in $B$, $\{\Psi_{k}, k \in [L]\}$ and $C$ remain unchanged during the optimization process, and so are activations in the diagonal matrices $\{D^i_k, i \in [n], k \in \{0,1,\ldots,L\}\}$. \autoref{fig:network_blocks} illustrate the described network. \\
% % Alternative explanation [WIP]: \\
% To proposed network is defined and initialized as follows. All layers are initialized with independant Gaussian distributions,
% \[
% \brackets{W_k}_{i,j}\sim\N(0, 2/m)~~,
% ~~\brackets{\Psi_k}_{i,j}\sim\N(0, 2/m),
% ~~\brackets{C}_{i,j}\sim\N(0, 2/d_x),
% ~~\brackets{B}_{i,j}\sim\N(0, 2/d_y)
% \]
% The only trained layers are $W_{[L]}$, while $\paren{B,C,\Psi_{[L]}}$ remain unchanged during training. 
% The activations $\{D^i_k, i \in [n], k\in [L]\}$ are computed based on the random weights of $\Psi_{[L]},B,C$ as follows,
% \[
% z^i_0 = [Cx_i]_+~~,~~z^i_k = [\Psi_k z_{k-1}^i]_+~~,~~  D_k^i = \mbox{diag}(z_k^i)~~~k=1,\ldots,L.
% \]
% Therefore do not change during training as well. \autoref{fig:network_blocks} illustrate the described network.

==> old_snapshots/related-2020-12-09.tex <==
\section{Related work} \label{sec:related}
% In this section we cover additional related works. \\
\textbf{Neural network overparameterization} has been extensively studied under different assumptions over the training data and network architecture.
For the simplified case of well-separated data, Ji et al.~\cite{ji2018risk} showed that a poly-logarithmic width is sufficient to guarantee convergence in two-layer networks, and Chen et al.~\cite{chen2019much} extended the result to deep networks using the NTRF function class~\cite{cao2019generalization}. For mixtures of well-separated distributions, Li et al.~\cite{li2018learning} proved that when training two-layer networks with width proportional to a high-order polynomial in the parameters of the problem with SGD, small train and generalization errors are achievable. Other common assumptions include Gaussian input~\cite{brutzkus2017globally,zhong2017learning,li2017convergence}, independant activations~\cite{choromanska2015loss,kawaguchi2016deep}, and output generated by a teacher-network~\cite{li2017convergence,zhang2019learning,brutzkus2017globally}. In our work, only a mild assumption of non-degenerate input is used.\\
overparameterization of special neural network is varied across the analysis of linear networks~\cite{kawaguchi2016deep,arora2018convergence,bartlett2018gradient}, smooth activations~\cite{du2018power,kawaguchi2019gradient}, and shallow networks~\cite{du2018power,oymak2020towards}. For deep linear networks, Kawaguchi~\cite{kawaguchi2016deep} proved that all local minima are global minima. Arora et al.~\cite{arora2018convergence} proved  trainability for deep linear network of minimal width, generalizing result by Bartlett et al~\cite{bartlett2018gradient} on residual linear networks. 
%\\
Neural networks with smooth activations were considered by 
Du and Lee~\cite{du2018power} showed that
in overparameterized shallow networks with quadratic activation, all local minima function are global minima. Kawaguchi and Huang~\cite{kawaguchi2019gradient}, that showed showed that when only the output layer is trained, i.e. least squares estimate with gradient descent, tighter bounds on network width can be achieved. 
Such assumptions over training and activations are rarely used in practice. 
%\\
Considering one-hidden-layer networks, Du et al~\cite{du2018gradient} showed that under the assumption of non-degenerate population Gram matrix, gradient-descent converges to a globally optimal solution.
Oymak and Soltanolkotabi~\cite{oymak2020towards} stated the current tightest bound on the width of shallow networks for different activation functions. For the ReLU activation, the bound we derive for deep networks is tighter. 
\\
We focus on the general setting of deep networks equipped with ReLU activation, as typically used in practice. 
Similar works~\cite{zou2018stochastic,du2019gradient,allen2019convergence,zou2019improved} require unrealistic overparameterization conditions, namely a minimal width proportional to the size of the dataset in the power of $(8,24,26)$~\cite{zou2019improved,allen2019convergence,zou2018stochastic}, and the depth of the network in the power of $(12$-$38)$~~\cite{zou2019improved,zou2018stochastic} or exponential dependency~\cite{du2019gradient}.
Our work improves current tightest bound~\cite{zou2019improved} by a factor of $O\paren{n^6 L^{11}}$, with a corresponding significant increase in convergence time.  
\\
\textbf{optimization landscape of deep networks} under different assumptions is an active line of research.
% Understanding the optimization landscape of ReLU networks under different assumptions is an active line of research.  
A few works showed that ReLU networks have bad local minima~\cite{venturi2018spurious,safran2018spurious,swirszcz2016local,yun2017global} due to "dead regions", even for random input data and labels created according to a planted model~\cite{yun2017global,safran2018spurious},
a property which is not shared with smooth activations~\cite{liang2018understanding,du2018power,soltanolkotabi2018theoretical}. Specifically, Hardt and Ma~\cite{hardt2016identity} showed
that deep linear residual networks have no spurious local minima
\\
\textbf{Training dynamics of ReLU networks} and their activation patterns were studied by few recent works~\cite{hanin2019complexity,hanin2019deep,li2018learning}.
% Few recent works studied the training dynamics of ReLU activation patterns~\cite{hanin2019complexity,hanin2019deep,li2018learning}. 
Hanin et al.~\cite{hanin2019deep} showed that the average number of patterns along the training is significantly smaller the the possible one and only weakly depend on the depth. We study a single random pattern, fully decoupled from depth.
Li and Liang~\cite{li2018learning} studied "pseudo gradients" for shallow networks, which are close in spirit with the fixed ReLU activations suggested by our work. They showed that unless the generalization error is small, pseudo gradients remain large, providing motivation for fixing activation patterns from generalization perspective. Furthermore, they showed that pseudo gradients can be coupled with  original gradients for most cases when the network is sufficiently overparameterized. \\


% with different analysis tools, 
% review additional related works of similar lines of research. \\
% Shallow neural networks with a teacher network - several works considered a 

% \begin{enumerate}
%     \item Towards moderate overparameterization:
% global convergence guarantees for training shallow neural networks - shallow (one training layer) with motivation to clost the theoretical-experimental gap. \\
% \item Fast Convergence of Natural Gradient Descent
% for Overparameterized Neural Networks - 2 layers \\
% \item Gram-Gauss-Newton Method: Learning Overparameterized Neural
% Networks for Regression Problems - like Du, using the least eigenvalue in bound for $m$. \\
% %\item Resnet-$1001$ layers - diracnet can fit, can we? \\
% \item Training (Overparametrized) Neural Networks
% in Near-Linear Time - larger $m$ but less iters since second order. Does assumption 3.1 always hold? huge neurons - so if we multiply by ratio of 1-2nd order, we're faster?\\
% \item Spurious Local Minima Exist for Almost All
% Over-parameterized Neural Networks- Smooth Activations. Due to the popularity of ReLU activations, a few works
% showed that ReLU networks have bad local minima (e.g., Swirszcz et al.[21]
% Zhou et al. [22], Safran et al.[23], Venturi et al.[16], Liang et al.[24]1
% ). One intuition why ReLU can lead to bad local minima is that it can create flat
% regions (“dead regions”) which are bad local minima. Intuitively, such flat
% regions may disappear if the activations are smoooth (this is indeed proved in
% Liang et al.[24] for special data).
% \item A Mean-field Analysis of Deep ResNet and Beyond:
% Towards Provable Optimization Via Overparameterization From Depth -  global convergence result for multilayer neural networks in the mean-field
% regime (infinite number of layers. We can relate that ultra-deep can work with our method only. 
% \item Over-parametrization for Learning and Generalization in
% Two-Layer Neural Networks - "open problem" - can be achieved with $nlog n$? 
% \item The Effects of Mild Over-parameterization on the Optimization
% Landscape of Shallow ReLU Neural Networks - conditions on $m$ so bad minimas become saddles.
% \item An improved analysis of training
% over-parameterized deep neural networks - another by Zou, improving the former -add to table.
% \item Proving the Lottery Ticket Hypothesis: Pruning is All You Need - small subnetwork for over-p one achieve similar results with much less params.
% \item Dynamic Graph: Learning Instance-aware Connectivity for Neural Networks - Modified relus (learned, in NAS context).
% \item Learning Overparameterized Neural Networks via
% Stochastic Gradient Descent on Structured Data - pseudo gradient, for generalization of 2-layer networks on well-clustered data.
% \end{enumerate}

==> plan.tex <==
\newpage


% \section{Status}
% \begin{enumerate}
%     \item New type of a neural network: nonlinearities are fixed per example (will refer as fixed-net as oppose to the regular relu-net)
%     \item Much tighter bound on network’s width (the tightest I’ve found, but depends on the dimension $d$ - see ‘questions’).
%     \item Elegant and cool proof.
% \end{enumerate}

\section{Action Items}
\begin{enumerate}
    \item Add my fixes to the tex and read again. [WIP]
    \item Move project to overleaf [DONE]
    \item Prepare a literature review on overparameterization. [WIP]
    \item Pick a suitable repo and implement fixed-net. Start with the ideas in the ‘empirical’ section.
\end{enumerate}
\section{Ideas}
\subsection{Theoretical}
\subsubsection{Motivation}
\begin{enumerate}
    \item  The number of activation regions in relu-netws doesn’t change much along the training~\cite{hanin2019deep}. Are relus bugs or features? 
    \item Fixed-net is equipped with the same nonlinearity, but no ‘dying relus’~\cite{lu2019dying}.
    \item Like \cite{allen2019convergence} theorem 5, can probably prove relation to NTK as corollary. Appears so, quite easily.
    \item Better avoidance of vanishing gradients?
    \begin{enumerate}
        \item Calculated the average number of ‘open’ relus on the train set (ResNet trained over ImageNet). It decreases with depth: from ~$60\%$ open in first layer to $20-30\%$ in last. Will try without skip connections as well. 
        \item Many try to remove slip connections from relu-nets. Usually ends with decreased accuracy and longer training time. 
        \item extending to $d_x,d_y$ is likely to remove the input's dimension from the bound. 
    \end{enumerate}
\end{enumerate}


\subsubsection{Properties}
\begin{enumerate}
    \item What is the network's memorization capacity? \\
    Inspired by the proof for theorem 3.1 of~\cite{yun2019small}, regions can be allocated after initialization, with concentration on the different combinations. Lemma 3 of the fixed-net notes can help. 
    \item Neural Tangent Kernel~\cite{jacot2018neural} \\ What properties can be derived for fixed-net ?
    \item Exponential moving average (EMA) \\
This is our strongest training-enhancement, increasing accuracy significantly for most tasks (possibly worth to publish based on those results alone) \\
Network A trains independently, and network B average its weights every $k$ steps: 
$$ W_B(t) \leftarrow (1-\alpha)W_B(t-k)+(\alpha)W_A(t) $$
Can we use the multi-linear form of the network to justify EMA as an ensemble method? The key is that the nonlinearities stay the same per example
(perhaps \cite{littwin2020collegial} can  help, modeling EMA as an ensemble)
\end{enumerate}

\subsubsection{Proof extensions}
\begin{enumerate}
    \item input and output sizes $(d_x,d_y)$ are different [relatively easy].
    \item Convolutional networks: can generalize to any network in the process of 2x runtime after implementing relu with 2 inputs.    
\end{enumerate}


\subsection{Empirical}
\begin{enumerate}
    \item Implement fully-connected fixed-net, and train back-to-back with relu-net, when both share the same initialization and hyper-parameters. 
    \begin{enumerate}
    \item Plot the usual stats and compare.
    \item If results are pleasing, same comparison with modern networks \item Train with EMA (see ‘properties’).
    \end{enumerate}
    \item Plot the fraction of active relus along training vs depth for relu-net, with and without skip connections (as motivation for fixed-net) [WIP]
    \item compare results with~\cite{li2019enhanced}
\end{enumerate}


\section{Open questions}
\begin{enumerate}
    \item Allen-zhu et al. \cite{allen2019convergence} achieved $m>Poly(n,L)$. \\
Why do we get a polynomial dependency on the dimension of the data $d$ ? what about different $(d_x,d_y)$? Answer: Allen received too dependency on the output's data - we will probably get the same if proving for $(d_x,d_y)$.
    \item On inference, does every new example need to first pass through the initial network in order to set it’s active gates? 
    \item What’s the rate of convergence compared to \cite{allen2019convergence}? answer: $\ell(W_{t+1}) - \ell(W_t) \leq -\frac{\eta\alpha^2 L}{4}\ell(W_t)$
    \item Can inference time be improved due to absence of Relus?
    \begin{enumerate}
    \item Can skip prior multiplications.
    \item On the other hand, active region indices need to be propagated with the batch, and additional matrices $\Psi_k$ are introduced.
    \end{enumerate}
\end{enumerate}

\section{text modifications}
\begin{enumerate}
    \item last page - add condition on $L$ and fix last equation. 
    \item change $||$ to norms + define that default is $l_2$ (remove the 2s?) -DONE (except lemma 3)
    \item define $\lambda(.)$
    \item figure to explain the architecture? DONE (\cite{allen2019convergence} have one.
\end{enumerate}
\section{Possible errors}
\begin{enumerate}
    \item We now handle the second term in (6), i.e: factor of $3$?
    \item sum of geometric series with negative ratio. Assuming $\eta$ makes the abs-ratio smaller than 1, we can bound with the first term. 
    \item and therefore
\[
    \ell(W_{t+1}) - \ell(W_t) \leq -\frac{\eta\alpha^2 L}{2}\ell(W_t) + \frac{\eta^2}{\beta^4L^2}\sum_{i=1}^n \nm{\Delta_{t,i}x_i}^2
\]
\asaf{
I got:
$\Lambda_i +\eta^2 a_i\leq -\frac{\eta\alpha^2 L}{2}$ \\
and therefore: \\
$\ell(W_{t+1}) - \ell(W_t) \leq -\frac{\eta\alpha^2 L}{4}\ell(W_t) + \frac{\eta^2}{\beta^4L^2}\sum_{i=1}^n \nm{\Delta_{t,i}x_i}^2$
}
\end{enumerate}
\nocite{*}
